SmartBook: AI-Assisted Situation Report Generation for Intelligence Analysts

Timely and comprehensive understanding of emerging events is crucial for effective decision-making; automating situation report generation can significantly reduce the time, effort, and cost for intelligence analysts. In this work, we identify intelligence analysts' practices and preferences for AI assistance in situation report generation to guide the design strategies for an effective, trust-building interface that aligns with their thought processes and needs. Next, we introduce SmartBook, an automated framework designed to generate situation reports from large volumes of news data, creating structured reports by automatically discovering event-related strategic questions. These reports include multiple hypotheses (claims), summarized and grounded to sources with factual evidence, to promote in-depth situation understanding. Our comprehensive evaluation of SmartBook, encompassing a user study alongside a content review with an editing study, reveals SmartBook's effectiveness in generating accurate and relevant situation reports. Qualitative evaluations indicate over 80% of questions probe for strategic information, and over 90% of summaries produce tactically useful content, being consistently favored over summaries from a large language model integrated with web search. The editing study reveals that minimal information is removed from the generated text (under 2.5%), suggesting that SmartBook provides analysts with a valuable foundation for situation reports

==> sections/0_Abstract.tex <==
\begin{abstract}
 %Emerging events require timely and comprehensive situation understanding for effective decision-making and response. Automated generation of situation reports can reduce the time, effort, and cost of intelligence analysts when preparing their official reports. 
Timely and comprehensive understanding of emerging events is crucial for effective decision-making; automating situation report generation can significantly reduce the time, effort, and cost for intelligence analysts. Through a formative study and collaborative design sessions, we identify intelligence analysts' practices and preferences for AI assistance in situation report generation to guide the design strategies for an effective, trust-building interface that aligns with their thought processes and needs. Next, we introduce SmartBook, an automated framework designed to generate situation reports from large volumes of news data, creating structured reports by automatically discovering event-related strategic questions. These reports include multiple hypotheses (claims), summarized and grounded to sources with factual evidence, to promote in-depth situation understanding. %Next, we propose SmartBook, an automated framework for generating situation reports: given large volumes of news data, produce a structured report with multiple hypotheses (claims) summarized and grounded to sources with factual evidence. %These reports are structured as a sequence of timespans, each consisting of major events.
 %SmartBook automatically discovers event-related strategic questions, with their grounded summaries promoting in-depth situation understanding. 
Our comprehensive evaluation of SmartBook, encompassing a user study alongside a content review with an editing study, reveals SmartBook's effectiveness in generating accurate and relevant situation reports that further benefit from human analyst refinement.
 %\textcolor{blue}{\textbf{TODO: Revanth - Change the below once we have user study results. They were criticized as 'over-claims' by reviewers.}} 
 %SmartBook offers an intuitive human-centric design that is amenable to intelligence analysis.  Qualitative evaluations indicate over 80\% of questions probe for strategic information, and over 90\% of summaries produce tactically useful content. Experts tend to add more information to the generated reports than they remove (under 2.5\% of existing tokens), indicating SmartBook provides analysts with a valuable foundation for situation reports. %SmartBook offers an intuitive and efficient approach to situation report generation, for reading and writing.

%\revanth{I now added a sentence related to strategic questions, but we're pretty constrained for space as CHI has a 150 word abstract limit}
%\heng{Can you add some emphasis on the unique functions of Smartbook including strategivally chapter and section/question generation? I think we need to add a bit intro to motivate the task.}

\end{abstract}

 %\footnote{We mourn the loss of our project contributor, Paul, who passed away before this paper's publication. His contributions were invaluable, and we honor his memory and dedication to the pursuit of knowledge.}


==> sections/10_Conclusion.tex <==
\section{Conclusion}\label{sec13}

In this work, we dive into the novel challenges and nuances of automated situation report generation, emphasizing the significant role of these reports in contributing to decision-makers' timely, in-depth understanding of emergent crises. Our approach, informed by a formative study and collaborative design, builds design strategies to address real-world intelligence analysts' needs. We have introduced \textbf{SmartBook}, an innovative framework crafted to generate situation reports with comprehensive, current, and factually-grounded information extracted from diverse sources. SmartBook goes beyond mere information aggregation; it presents chronologically-ordered sequences of topic-summarized events extracted from news sources and placed into a UI layout structure that aligns to the workflow of intelligence analysis. By involving analysts at each stage of SmartBook's conceptualization from design through evaluation, we pave the way for a more cohesive and productive analytical workflow. Our user study, with ten intelligence analysts and two decision-makers, validated SmartBook's effectiveness in providing grounded and easy-to-digest information with its intuitive interface. Both intelligence analysts and decision-makers found SmartBook to be usable, feasible to integrate into operational environments, and trustworthy.



%In this paper, we present the novel task of automated situation report generation, which is pertinent for timely and scalable complex event understanding of emergent crises. This problem formulation differs from the traditional multi-document news summarization domain in that it requires comprehensive, broad coverage of important information, which is to be presented in a structured format that is spread across a timeline.
%In addition, the vast amount of information needs to be organized into chapters and sections with a strategic structure to facilitate analysis and planning. To address these challenges, we propose \textit{SmartBook}, a generalizable framework for clustering news topics and summarizing news claims automatically. SmartBook offers automated generation of situation reports as an initial draft consolidating information to assist analysts, not to replace them. 

%For future work, we aim to explore the following avenues to improve the reliability and expand the scope of SmartBook:

%\begin{itemize}
  %  \item \textbf{Controlling the bias of sources:} To control bias in SmartBook, we will cross-check information from various news sources with differing angles, levels of detail, and interpretations, and also consider independent sources from the left, center, and right to identify alternate perspectives and hypotheses. \\
%    \item \textbf{Adding more languages:} By incorporating news articles from various languages, we plan to capture diverse perspectives, insights, and information on global events, while also enabling analysts to understand local customs, cultures, and nuances that influence event interpretation, ultimately presenting a more comprehensive and accurate picture. \\
 %   \item \textbf{Verifying the extracted claims:} Since situation reports inform strategic planning, we will provide a trustworthiness verification score for each SmartBook claim to ensure accuracy and prevent misguided actions, with lower scores indicating the need for further analyst oversight before final report inclusion.
%\end{itemize}

==> sections/1_Intro.tex <==
\section{Introduction}\label{sec1}

%\heng{We should also talk about criteria for a good situation report - use the bullets in page 6 of these slides: https://blender.cs.illinois.edu/ALTA\_NLP\_SmartBook\_HengJi.pdf}

In today's rapidly changing world, intelligence analysts face the constant challenge of staying informed amidst an overwhelming influx of news, rumors, and evolving narratives. Currently, intelligence analysts prepare \textit{situation reports}, about the state of affairs, potential risks or threats, and perspective, with recommended actions \cite{world2020coronavirus,world2022emergency}. The downstream consumers of these reports (general public, decision-makers, and stakeholders) are not just looking for raw information; they are seeking clarity, context, and actionable insights. However, these reports, being manually crafted, come with limitations: they are time-consuming~\cite{national2019decadal}, might exhibit biases~\cite{biases1, belton2020cognitive}, and may be restricted due to the large volume of information they must process~\cite{doggette2020information, overload1}. %Most importantly, the process of generating and consuming these reports is far from optimized for the user (analysts), impacting its downstream recipients. 
Intelligence analysts spend extensive time sifting through vast and complex data sources~\cite{golson2018resist, national2011intelligence} ({\em e.g.,} social media rumor propagation, news outbreak, background statistics, domain expert opinions, etc.), and readers often grapple with information that's either too dense or not sufficiently comprehensive. Given the sheer volume of information, it is challenging for analysts to do deep analysis and critical thinking, to be able to formulate strategic questions and generate insights.

We hypothesize that automatic situation report generation can bridge the gap in reading and writing intelligence information. Existing summarization approaches~\cite{fabbri-etal-2019-multi, abdi2017query, li2014improving} generate plain-form text and do not yield the details, structures, and high-level strategic information to support decision-making for the downstream consumer. In particular, current Large Language Model (LLM) based approaches such as GPT-4/ChatGPT~\cite{openai2021gpt35} may return no answers or incorrect answers to user questions as they do not update information in real-time and lack fact-checking mechanisms ({e.g.,} Table~\ref{tab:chatgpt}). 

To establish a basis for the automated generation of situation reports, we initially carried out a formative study\footnote{All study protocols were approved by our institution's IRB.} (see \S{\ref{sec:formative_study}}) to grasp the standard practices in situation report creation and intelligence analysts' expectations from AI-driven systems. Our findings reveal that analysts are open to AI assistance, seek clarity in AI operations, and vary in their desire to control the AI system. To further comprehend the composition process of situation reports, we augmented the initial study's findings with collaborative design sessions, aiming to define practical design strategies and recommendations, particularly on how intelligence analysts navigate, research, and write their reports. On a high level, we infer (in \S{\ref{sec:collaborative_results}}) that the system interface must visually align with analysts' sequential thought processes, provide transparency of information flow to build trust, and enable analysts to have some level of control over the AI tool's processes. These conclusions consequently guided the design strategies (in \S{\ref{sec:design_strategies}}) for automating the generation of situation reports.

%\textcolor{blue}{\textbf{TODO: Revanth - Summarize design recommendations brought forward in collaborative study.}}

\input{tables/chatgpt}


% However, real-world situation intellgence reports that policymakers and subject matter experts rely on for decision-making require detailed, real-time information. For example, recent expert-written situation reports \cite{bowen2022russia} on the Russia-Ukraine crisis, published by the United Nations and the U.S. Congressional Research Service, aggregate critical information on social conditions and history as background; onset of the military invasion; development of subsequent military operations; economic, political, and humanitarian ramifications; and present an outlook forecast – in over twenty dense pages. Automating the generation of situation reports \textit{goes beyond} increasing the volume of retrieved, relevant news sources \cite{brody-kantor-2011-automatic} and the length of generated summaries. It \textit{extends to} maintaining a structured organization ({e.g.,} chapters and sections) for ready access and understanding of complex events, in support of strategic planning. As such, the current application of AI techniques to situation analysis and report generation is far from mature.  

\begin{figure}[t]
\includegraphics[width=\textwidth]{figures/SmartBook_example.png}
\caption{Figure showing an example from SmartBoook for the Ukraine-Russia Crisis. SmartBook is organized on a timeline, with 2-week time spans containing chapters and corresponding sections. The section headings are strategic questions and each section content consists of a grounded summary with links to relevant claims, each highlighted for factual evidence and knowledge elements. The entities and events (along with corresponding types), which comprise the associated knowledge elements, are highlighted in red and blue respectively.} 
\label{fig:1}
\end{figure}

Building on the foundation set by the formative study and collaborative design, we present \textbf{SmartBook}, a framework designed to assist human analysts who author situation reports. SmartBook ingests data from multiple sources to generate a comprehensive report with information updated on a regular basis. The framework automatically discovers questions important for situation analysis and gathers salient information for generating the report. For all questions about a major event, the report contains summaries with tactical information coming from relevant claims, presented with local context and links to source news articles. SmartBook structures data in a manner that mirrors current intelligence analyst workflows--breaking down events into timelines, chapters, and question-based sections. Each section contains a grounded query-focused summary with its relevant claims. This intuitive structure facilitates easier assimilation of information for both reading and writing. Designed with a human-centered approach, our goal is to augment the capabilities of human analysts rather than replace them. Figure \ref{fig:1} shows an example from SmartBook for the Ukraine-Russia crisis, with the structured hierarchy of timespans, chapters, and corresponding sections.


In our comprehensive evaluation of SmartBook, we conducted two complementary studies: a user study (in \S{\ref{sec:usability_study}}) for assessing usability and interaction, and a content review (in \S{\ref{sec:content_review_study}}) for examining the quality of text summaries. The user study, involving intelligence analysts and decision-makers, focused on key research questions to explore SmartBook's usability, intuitiveness, and effectiveness in situation report generation. Participants engaged in semi-structured interviews and post-study questionnaires, reflecting on their experience with the system. The content review complemented this by assessing the readability, coherence, and relevance of SmartBook-generated reports, including an editing study where an expert analyst revised the summaries until they met their standards of acceptability. This process aimed to determine the viability of using SmartBook as a tool for creating preliminary drafts in analytical settings. %Results indicated that SmartBook seamlessly integrates into analysts' workflows, mirroring their conventional report generation processes with an intuitive and user-friendly interface. 
The system's generated reports were noted for their accuracy and relevance, enhancing efficiency in report generation. Furthermore, the editing study with an expert analyst suggested that while SmartBook lays a solid foundation, it benefits from human refinement. Overall, SmartBook emerged as a robust tool for intelligence analysis, balancing automated efficiency with the need for human expertise.

%Cut down and add in the content review.

%\textcolor{blue}{\textbf{TODO: Daniel - Add a brief paragraph showing the overall flow of the paper, i.e. formative study guides collaborative design guides design strategies guides Smartbook, and then system + content evaluation studies}}

 %\textcolor{blue}{\textbf{TODO Revanth: add in sentence, per Agathe, that our approach is presented for how to proceed in integrating an AI into the task of situation report generation, the approach and insights can be applied more broadly to other tasks. In other words, this is not a one-off exemplar.}}

% As a case study, we consider the case of automatic situation report generation for the Ukraine-Russia crisis. This scenario is particularly challenging, given the complexity of the conflict, the politicization of the issue, and the need to regularly update the reports as the situation evolves. 

%Our proposed automatic situation report is created from a corpus of news articles and is organized along a timeline, with new timespans added as the conflict progresses. Each timespan covers a 2-week period and each major event identified within that period is the basis for a separate chapter. Each chapter is further subdivided into sections corresponding to the automatically identified strategic questions that are relevant to the chapter event.  Each section contains a grounded query-focused summary with its relevant claims. Figure \ref{fig:1} shows an example from SmartBook for the Ukraine-Russia crisis, with the structured hierarchy of timespans, chapters and corresponding sections.


%Our contributions, centered around enhancing user experience and promoting effective human-computer collaboration in the intelligence analysis space, can be summarized as follows:
The contributions of this work are as follows:
\begin{itemize}
    \item A comprehensive formative study and collaborative design process for identifying the design strategies to guide the automated generation of situation reports.
    \item \textbf{SmartBook}, an automated framework that generates comprehensive, up-to-date situation reports from various sources and presents them in an intuitive and user-friendly manner. It identifies critical strategic questions, ensuring that downstream readers receive targeted, relevant, and evidence-grounded information to aid their decision-making processes.
    \item A user study with 10 intelligence analysts and 2 decision-makers investigating the usability of the system.
    \item A content review to grade the quality of the information generated, along with an editing study to understand how viable SmartBook is for producing preliminary first drafts.    
    %\item Through both quantitative and qualitative evaluation focusing on situation report generation for the Ukraine-Russia crisis, we demonstrate that SmartBook is not just technologically robust but also meets the usability and informativeness expectations of expert analysts, proving vital for strategic planning.
    %\item In terms of providing actionable intelligence to users, we show that SmartBook outperforms a web search $+$ large language model approach (akin to Bing + ChatGPT) by up to 9\% in terms of relevance and strategic value of the information presented. 
    %\item \textcolor{blue}{Finally, we show results from a study on a senior expert intelligence analyst performing the task of situation report generation, by using SmartBook's output as a preliminary first draft.}
    \item A publicly accessible interface for SmartBook and underlying code to foster collaboration, feedback, and further innovation in the intelligence analysis domain.
\end{itemize}

%\item We identify an exciting new problem domain and task formulation of \textit{automated situation report generation}, which aims to assist human analysts, not replace them.
    %\item We propose \textsc{\textbf{SmartBook}}, an automated framework that generates comprehensive, up-to-date situation reports from various sources, by discovering critical strategic questions and grounding the report with trustworthy factual evidence.
    %\item We quantitatively and qualitatively evaluate our automatic situation report generation approach for the Ukraine-Russia crisis and demonstrate that SmartBook is well-received by expert analysts in terms of informativeness and effectiveness for strategic planning.
    %\item We show that SmartBook outperforms a web search $+$ large language model based generation approach (akin to Bing + ChatGPT) by up to 9\% in terms of relevance and strategicness of information presented. 
    %\item Finally, we contribute a publicly accessible UI\footnote{\url{https://blenderdemo.com/smartbook}} and code\footnote{\url{https://github.com/blender-nlp/SmartBook}} for SmartBook so that others can explore and improve upon these.
    
%\wordcount

==> sections/2_Related_Work.tex <==
\section{Related Work}

\subsection{AI for Intelligence Analysis}

% Expand existing discussion on how AI has been used to help intelligence Analysts and how SmartBook is different from these approaches

%\textcolor{red}{need to extend each step in the first paragraph}

% \textcolor{blue}{Situation reports are pivotal in intelligence analysis, often requiring a synthesis of complex, and sometimes conflicting data from various sources. The introduction of Artificial Intelligence (AI) tools like SmartBook promises to revolutionize this process, offering an automated framework for report creation, which can serve as a foundational draft for intelligence analysts. In this section, we delve into the current landscape of AI in intelligence analysis and position SmartBook's innovation in this space.}

AI has ushered in a new era for intelligence analysis, as traditional methods can be often tedious and time-consuming. AI, however, can manage vast data sets and swiftly analyze information, ensuring accurate and timely insights. The intelligence analysis begins with data collection and ingestion, where automated tools play a pivotal role in efficient categorization and storage as highlighted by studies~\cite{stottlemyre2015humint, billman2006collaborative,pohl2012automatic}. These tools gather data from diverse sources, simplifying access for further analysis.
%AI has ushered in a new era for intelligence analysis. Traditional methods, though efficient, are often tedious and time-consuming. AI, however, can manage vast data sets and swiftly analyze information, ensuring accurate and timely insights. The initial step in intelligence analysis involves data collection and ingestion. As highlighted by studies like ~\cite{stottlemyre2015humint, billman2006collaborative,pohl2012automatic}, automated tools are crucial for this phase. They ensure a streamlined categorization and storage of data from an array of sources, making it easily accessible for subsequent processing. 
%\heng{maybe give some stats about how much time human analysts usually need to spend on drafting a report, and they can only update the report once every two weeks. You can check some wording in my slides: \url{https://blender.cs.illinois.edu/ALTA\_NLP\_SmartBook\_HengJi.pdf}}
In the domain of data visualization and examination~\cite{prunckun2010handbook}, AI significantly enhances the ability to discern complex data patterns, aiding analysts in drawing meaningful inferences. Furthermore, the assessment of evidence reliability is crucial. AI-driven tools can systematically evaluate information credibility, ensuring the use of verified data~\cite{barnes2016making, toniolo2014making}. Further, they can examine the depth and accuracy of insights, verifying the validity of intelligence reports~\cite{brody2011automatic}.
%The realm of data visualization and inspection has also benefited immensely from AI. Tools recommended by Prunckun et al. ~\cite{prunckun2010handbook} aid analysts in visualizing intricate data patterns, thereby aiding the drawing of meaningful conclusions. It's imperative to determine the reliability of the sourced evidence. AI-driven tools, as suggested by Barnes~\cite{barnes2016making} and Toniolo et al. ~\cite{toniolo2014making}, serve this purpose by systematically evaluating the credibility of the information, ensuring analysts work with verified and reliable data. ~\cite{brody2011automatic} introduced tools that scrutinize the depth and accuracy of insights, certifying the produced intelligence reports' validity.
%\heng{here maybe add a sentence to say that we partially solved this problem by making sure claims are carefully extracted and grounded into source, and thus 98\% of the information in our report draft is accurate and thus users can spend minimal time on inspection}
AI innovations, such as those exemplified by HITIQA~\cite{small-etal-2004-hitiqa-scenario}, have facilitated scenario-based question answering, essential for dissecting specific situations and deriving precise insights. This approach is crucial in intelligence analysis, where generating potential hypotheses is a key aspect~\cite{heuer1999psychology, cerutti2018cispaces}. While these developments represent significant progress, challenges persist. Studies~\cite{van2020improving,xia2019trace,pirolli2005sensemaking,pioch2006polestar,toniolo2023human} point out that current tools often require extensive crowdsourcing or necessitate human-machine collaboration for report drafting, highlighting the need for further improvement in this area.

%AI innovations have also paved the way for scenario-based question answering, as demonstrated by HITIQA ~\cite{small-etal-2004-hitiqa-scenario}. Such frameworks are instrumental in dissecting specific situations and obtaining precise insights. Further, the generation of potential hypotheses is a core component of intelligence analysis. ~\cite{heuer1999psychology, cerutti2018cispaces} have advanced this process, offering a range of probable scenarios for analysts to consider. However, despite these advancements, challenges remain. Current tools, ~\cite{van2020improving, xia2019trace} point out, often demand extensive crowd-sourcing or necessitate human-machine collaborations for report drafting, as evidenced by research from~\cite{pirolli2005sensemaking, pioch2006polestar, toniolo2023human}.

%\textcolor{blue}{Artificial Intelligence (AI) tools significantly augment Intelligence analysts' ability to collect, process, analyze, and infer insights from the data.Automatic tools automate the process of collecting and ingesting data from various sources, ensuring that the information is categorized and stored for easy retrieval. }
%Automatic tools assist intelligence analysts in data collection, data inspection and visualization~\cite{prunckun2010handbook}, evidence credibility assessment~\cite{toniolo2014making,barnes2016making}, scenario-based question answering~\cite{small-etal-2004-hitiqa-scenario}, hypotheses generation~\cite{heuer1999psychology, cerutti2018cispaces}, and quality valuation~\cite{brody2011automatic}.
SmartBook brings in a significant advancement in automated situation report generation. SmartBook aims to produce initial report drafts, allowing analysts to channel their energies on critical thinking and comprehensive assessments. Additionally, the system's integration of a large language model aids in topic discovery, navigating the longstanding issue of analysts being unaware of unknown factors. By generating strategic questions for varying events, it guides analysts towards previously unseen patterns, prompting the exploration of new hypotheses, even when confronted with contradictory information. In an age where data inundation is a constant challenge for intelligence analysts, tools like SmartBook offer not just relief, but a pathway to enhanced efficiency and deeper insights. This research underscores the promise of SmartBook, positioning it as a significant milestone in AI-assisted intelligence analysis. 
%\revanth{SmartBook can obtain news articles for any given time periods that correspond to the event (that is how Google News supports it), but we don't formally evaluate it.}
%\heng{do we have any formal evaluation about how timely the information in smartbook is?}

\subsection{Multi-Document Summarization}
Multi-document summarization aims to extract critical information across multiple documents into a few-sentence summary~\citep{fabbri-etal-2019-multi, abdi2017query, li2014improving, xiong2018multi, abdi2018qmos, abdi2018machine, deyoung2021ms2}.
Large Language Models (LLMs) have also shown unprecedented ability to generate summaries~\citep{zhang2023extractive,zhang2023benchmarking, yang2023exploring, zhang2023enhancing, wang2023zero, zeng2023meta}.
SmartBook differs from these summarization tools with its structural narratives, its focus on situational intelligence, and its automatic event-related question discovery.
First, the current summarization methods lack the organizational structure needed for intelligence situation reports, which require synthesizing diverse data points into a coherent narrative. 
SmartBook, by contrast, generates inherently structured reports that are broken down into time spans, major events, strategic questions, and their grounded summaries.
This layered structure, reminiscent of a book, provides a comprehensive view and intuitive navigation through the complex scenario being analyzed.
Second, while news summarization aims to provide a condensed version of events, SmartBook not only states what happened but also explores multiple aspects including implications, potential trajectories, and strategic importance of these events.
Third, previous query-based methods rely on human effort to identify important events as guidance or prompts, while SmartBook introduces an innovative mechanism to discover pertinent event-related questions automatically, allowing the system to probe deeper into events to offer users richer insights. 

\begin{comment}
The challenge of synthesizing information from multiple sources is a long-standing one in the fields of information retrieval and natural language processing. SmartBook builds upon these traditions but adapts them to the nuanced requirements of situation reports for end-user usage.

Automatic news summarization has been the focus of significant research~\cite{mani2001automatic}, aiming to help readers quickly grasp the main points from vast daily news articles.  Early methods relied heavily on extracting salient sentences from the articles based on word frequency and location~\cite{luhn1958automatic}. Later efforts, like TextRank~\cite{mihalcea2004graph}, use graph-based models to rank sentences. Following work on knowledge-enhanced summarization extracts useful information with prior knowledge, such as sentence similarity~\cite{wan2008exploration}, semantic role \citep{yan2014srrank, khan2015framework, khan2015genetic, alshaina2017multi}, Yago knowledge base~\citep{baralis2013multi}, and dependency parsing~\cite{kurisinkel2017abstractive}. While effective for generating short news summaries, these methods lack the depth and organizational structure needed for intelligence situation reports, which require synthesizing diverse data points into a coherent narrative. SmartBook, instead, identifies events, actors, and their relationships, organizing these into a structured report.

Summarizing multiple news articles into an situation analysis report is a new type of multi-document summarization~\cite{fabbri-etal-2019-multi, abdi2017query, li2014improving, xiong2018multi, abdi2018qmos, abdi2018machine}, which aims to extract critical information across multiple documents with particular guidance, such as sentiments~\citep{abdi2018machine}, queries \citep{abdi2018qmos}, and document structures~\citep{deyoung2021ms2}, into a few-sentence summary~\citep{fabbri-etal-2019-multi}. By contrast, the guidance in our query-based situation report summarization is identified and organized event knowledge in real-world scenarios (e.g., COVID and Russia-Ukraine Crisis). SmartBook’s goal expands past information summarization to the creation of an in-depth situation report based on multiple data streams. What sets SmartBook apart from traditional summarization tools is its focus on `situational intelligence'. While news summarization aims to provide a condensed version of events, SmartBook not only states what happened but also explores multiple aspects includiong implications, potential trajectories, and strategic importance of these events.

Large Language Models (LLMs) have set benchmarks in various natural language processing tasks, with their unprecedented ability to generate human-like text. Specifically, for text summarization, they have been used to produce extractive \cite{zhang2023extractive}, abstractive \cite{zhang2023benchmarking}, query-based \cite{yang2023exploring}, cross-document \cite{zhang2023enhancing} and cross-lingual summaries \cite{wang2023zero}. 
%However, SmartBook rises above conventional LLM-driven summarization by tailoring its capabilities to the domain of situation report generation.
Unlike generic LLM summaries that are linear and often lack detailed organization, SmartBook generates reports that are inherently structured, broken down into timespans, major events, strategic questions, and their grounded summaries. This layered structure, reminiscent of a book, provides a comprehensive view and intuitive navigation through the complex scenario being analyzed. Traditional summarization with LLMs, even if query-based, relies on external prompts. In contrast, SmartBook introduces an innovative mechanism to discover pertinent event-related questions automatically, allowing the system to probe deeper into events to offer users with richer insights. \heng{here we need to talk about LLM hallucination problem and how smartbook solves that problem}

%Our work is closely related to knowledge-enhanced summarization, which extracts useful information with prior knowledge, such as sentence similarity~\cite{wan2008exploration}, semantic role \citep{yan2014srrank, khan2015framework, khan2015genetic, alshaina2017multi}, Yago knowledge base~\citep{baralis2013multi}, and dependency parsing~\cite{kurisinkel2017abstractive}. 
%Nevertheless, the above methods do not meet the requirements for situation reports, as their outputs are typically short and do not organize events described in multiple documents, unlike SmartBook.
\end{comment}
%\subsection{AI-Assisted Writing}


%\revanth{As per reviewer comments, this section needs to be rewritten to focus less on `collaborative writing/co-authoring` as SmartBook doesn't really provide iterative report generation, to be classified as co-authoring or collaborative.}
%AI-assisted writing~\cite{WangACL2019,Wang2020,selfcollaboration2023,cardon2023challenges} is a rapidly growing field in human-computer interaction research. In recent years, researchers have explored various approaches to develop AI systems that can assist users in writing tasks. AI-assisted writing tools have demonstrated benefits to a variety of end-users, like academics~\cite{gero2022sparks}, screenwriters~\cite{mirowski2023co} and developers~\cite{chen2021evaluating}. CoAuthor~\cite{lee2022coauthor} crafts a dataset that encapsulates the rich interactions observed between multiple writers and instances of GPT-3 over numerous writing sessions, thereby highlighting the efficacy of AI in fostering collaborative writing endeavors. In the area of automated story-writing~\cite{klein1973automatic}, attempts such as Creative Help~\cite{roemmele2015creative}, Writing Buddy~\cite{samuel2016design} and WordCraft~\cite{yuan2022wordcraft} aid the user in producing full stories with creative control throughout the process. More recently, with humans struggling to identify text as being machine generated ~\cite{wahle2022large}, concerns have been raised about academic integrity~\cite{perkins2023academic} and plagiarism\cite{wahle2022identifying} when using AI-assisted writing tools. In light of the ongoing developments in the AI-assisted writing, SmartBook introduces a unique automated framework designed specifically for generating situation reports for intelligence analysts. While the existing body of work predominantly focuses on augmenting creative and collaborative writing, SmartBook seamlessly integrates with analysts' workflows, emphasizing efficiency, analytical depth, and breadth. 

%\subsection{Structured Report Generation in other domains}

%\textcolor{blue}{Structured report generation has become pivotal across a multitude of domains, driven by the quest to extract meaningful insights from vast datasets. Medicine is one of the domains where structured report generation has gained significant traction. Natural language processing (NLP) and computer vision algorithms have been used to generate radiology reports by analyzing medical images \cite{kisilev2015medical, monshi2020deep}. In the finance sector, firms leverage machine learning and AI models to sift through vast amounts of financial data to produce concise, structured quarterly or yearly financial reports~\cite{}. }

%\textcolor{blue}{In the domain of meteorological reporting, AI's application spans from predicting weather patterns to offering detailed narratives~\cite{leon2002intelligent, sripada2014case}. Sports analytics, on the backdrop of rising demand, has moved towards converting raw match data into post-match summaries, aiding analysts and enthusiasts alike in deciphering game dynamics~\cite{araujo2021artificial, bhatnagar2022systematic}. Similarly, the urgency of environmental concerns has spurred the use of satellite data integrated with machine learning algorithms, producing environmental reports on critical subjects such as deforestation and urbanization~\cite{van2014environmental, piedelobo2018hidromap}.}

%\textcolor{blue}{Lastly, the corporate sector, especially e-commerce, has not remained untouched. Businesses, overwhelmed with vast pools of data, employ AI-driven tools to decode this data and produce structured reports. These reports offer pivotal insights into sales trends, customer behaviors, and market dynamics, thus aiding decision-making processes~\cite{negash2004business}. Such extensive applications across various sectors underscore the potential of AI-driven tools, with SmartBook aiming to assist intelligence analysts by presenting them with thorough situation reports.}

%In the medical field, algorithms analyze medical imagery to craft detailed radiology reports. 
%The finance sector employs machine learning to process immense financial data, thereby automating the creation of concise quarterly or yearly reports. Weather forecasting now integrates sophisticated AI algorithms, going beyond mere statistical predictions to craft detailed daily weather narratives

%\textcolor{blue}{Similarly, the urgency of environmental concerns has spurred the use of satellite data integrated with machine learning algorithms, producing reports on critical subjects such as deforestation and urbanization . The business analytics domain, overwhelmed by the sheer volume of its data, leans on AI tools to generate reports offering insights into diverse facets like sales trends and customer behaviors. Such extensive applications across various sectors underscore the potential of AI-driven tools, with SmartBook aiming to assist intelligence analysts by presenting them with thorough situation reports.}

 %and the summary is a comprehensive detailed report supporting in-depth analysis for decision-making and responses.

%\textcolor{blue}{
%\begin{itemize}
 %   \item \textit{Information Overload}~\cite{doggette2020information, overload1}: Analysts are often swamped with more data than they can efficiently process. Distilling relevant information from vast amounts of data is time-consuming and challenging.
 %   \item \textit{Disinformation and Misinformation}~\cite{golson2018resist, benzie2022artificial}: Not all information sources are reliable. Analysts must constantly be on the lookout for false or misleading information, whether intentional (disinformation) or unintentional (misinformation).
  %  \item \textit{Cognitive Biases}~\cite{belton2020cognitive, biases1}: Analysts, like all humans, are susceptible to cognitive biases. These biases can affect the interpretation of information, potentially leading to inaccurate assessments.
   % \item \textit{Time Pressure}: Especially in crisis situations, there's pressure to produce reports quickly, which can lead to oversights.
    %\item \textit{Complexity and Ambiguity}: Real-world situations can be complex, with many interconnected factors. Sometimes, the information available is ambiguous or contradictory, making definitive conclusions challenging.
%\end{itemize}
%}







==> sections/3_Formative_Study.tex <==
\section{Formative Study}
\label{sec:formative_study}
To gain an operational understanding of the range of processes that take place during intelligence analysis and generating situation reports, we conducted a formative study to gather information on: (1) regular practices in authoring situation reports and (2) general needs and expectations from intelligence analysts for AI-driven systems. Below, we start with a brief description of situation reports to provide background and then proceed with specifics on the formative study.

%\heng{I think the study description section can benefit from more concrete writing. maybe even attach the assessment guidelines etc. in appendix}

\subsection{Background}
\label{sec:situation_report_background}
%\textcolor{blue}{\textbf{TODO: Daniel - Needs some explanation (maybe at the beginning of Section 3) on why this situation report overview section is here.}} \revanth{Is this `our understanding' of what situation reports are and how they are generated, based on the formative study?}
%\daniel{I've added a short sentence below; however, the study task also describes that a component of the formative study is to understand what situation reports are and how they're created.}\item \textcolor{blue}{\textbf{I'll edit above at start of section.}}
A situation report is a document produced by an intelligence analyst to disseminate critical information. The report typically focuses on a specific issue or topic and provides a comprehensive overview of the information available on that topic. Intelligence analysts draft situation reports through a meticulous and systematic approach that begins with the collection of information from diverse sources, such as news articles, broadcasts, and potentially classified intelligence feeds. Once gathered, they prioritize the verification of this data, procuring reliable sources to ascertain accuracy. The subsequent analysis phase involves delving deep into the raw data to discern patterns, motivations, and implications, often requiring specialized knowledge or technical expertise. Post-analysis, the synthesized information is integrated into a cohesive narrative, emphasizing relevance and urgency, resulting in a clear, concise, and actionable report that communicates the prevailing situation to stakeholders. %Generating a situation report can take from 30 minutes to 3 hours, depending on the urgency, scale and complexity of the given situation.
The ultimate goal of such reports from intelligence analysts is to support downstream readers (i.e., consumers of the reports such policy-makers, government officials, and military personnel) in keeping track of developments by providing them with the time-critical, necessary information to make informed decisions and take appropriate actions.

\subsection{Method}
\label{sec:formative_method}
\subsubsection{Recruitment}
\input{tables/intelligence_analyst_demographic}
For the formative study, we targeted individuals with experience in government and military roles. We distributed a pre-screening survey to ascertain their background in creating situation reports. Participants qualifying for the study were either experienced intelligence analysts or had a minimum of one year of equivalent experience. The final group comprised 10 military personnel from different branches, as shown in Table \ref{tab:analyst_demographic}. Their experience in intelligence report writing varied between 1 and 10 years.

%\textcolor{blue}{In our study\footnote{The study protocol was approved by our institution's IRB.}, we engaged with individuals who have served, or are currently serving, in various capacities within government, including the military. To identify potential participants, we disseminated a pre-screening survey focused on eliciting information about their prior experience in generating situation reports. Those who qualified for our study self-identified as experienced intelligence analysts (or with 2 years of equivalent experience). Our final participant pool consisted of 10 individuals: 10 armed forces personnel from various branches of the military. As detailed in Table \ref{tab:analyst_demographic}, the range of their experience in intelligence report authoring spans from 2 - 10 years.}

%{\textcolor{red}{\textbf{need to spell out what``ML Prof.'' and the values 1,2,4 refer to in caption of Table 2  -- Clare}}

 %\heng{do we need to provide more details who these analysts are? which agencies are they from?}
%\daniel{In the interest of privacy, especially for military personnel, we don't particularly require additional information. From a reviewer's perspective + paper contribution, the granularity in military demographic details don't add more value per say. }
%\heng{maybe we should also add more details on why we choose them as our users - first, we choose ukraine crisis as a case study because it's a complex situation and we need AI to identify important information and generate strategically important questions and answers; so we choose users from the military for this study? also we need to emphasize our techniques are not limited to military domain, we also have done other case studies on earthquake, dipomacy, etc.}
%\daniel{For an HCI study, we come from an inductive approach. Meaning, we don't begin with a tool or a hypothesis, rather a user group. Therefore, a deductive approach common in NLP, where we have the tool, and identify the correct user group to evaluate against is not used. It is true, that our techniques are not limited to the military domain; therefore, this is within the discussions + future work section, where we can discuss the technology is generalizable.}

\subsubsection{Study Task} Over a two-week period, semi-structured interviews were conducted to examine two key areas: Authoring Experience and AI-Assisted Tools in situation report generation. The Authoring Experience section focused on participants' personal experiences in creating intelligence reports, including their methodologies, challenges, and key aspects of their authoring process. The AI-Assisted Tools section explored their understanding, attitudes, and recommendations regarding AI use in professional settings.

%The interview sessions, conducted over 2 weeks, adhered to a semi-structured format, systematically exploring two aspects of generating situation reports: Authoring Experience and AI-Assisted Tools. In the Authoring Experience segment, we delved into the participants' own experiences with creating intelligence reports, exploring their processes, notable challenges, and focal points in their authoring journey. The AI-Assisted Tools component concentrated on participants' understanding, perspectives, and suggestions of using AI, including their general attitudes towards AI, and its integration into their professional practices.}

The interviews began with open-ended questions to encourage unrestricted responses, followed by targeted inquiries for deeper insight into their report authoring perspectives. Each 60-minute session, conducted via video conferencing, allowed participants to extensively share their experiences and views. Compensation ranged from \$25 to \$35 per hour, reflecting participants' levels of experience.
%Each interview commenced with broad, open-ended questions, designed to minimize constraints on participant responses, while probing the topics that arose naturally in follow-up inquiries to deepen our understanding of their perspectives on authoring reports. This approach allowed participants to elaborate at length on their experiences and views. Each session spanned 60 minutes and was conducted via video conferencing, ensuring a thorough and consistent exploration of the topics raised by participants. Participants were compensated \$25 - \$35 per hour, commensurate with their experience.}
%\item \textcolor{red}{\textbf{I switched 'themes' to 'topics' since the term 'themes' is used below for content that is discovered and coded.  -- Clare}}

\subsubsection{Analysis Procedure}%\revanth{I agree with Agathe here. We might need to show the themes/codes. Should we add in that flowchart that you had in the slides?}
\label{sec:formative_analysis}
The interview data analysis employed an inductive method, abstaining from any pre-existing theories or hypotheses. Two members of the research team concurrently examined the same data segments and noted their findings independently. This stage highlighted emerging \textit{themes} related to analysts' perceptions and expectations of AI-assisted authoring tools, such as trust, efficiency, and interaction. A thorough coding of the interview transcripts followed, aiming to systematically pinpoint these themes. This entailed a repetitive process of code development and adjustment as the team navigated the transcript collection. To ensure accuracy and thoroughness, periodic cross-checks were conducted by two coders.

%The analysis of the interview data followed an inductive approach, in which our observations and data were collected without preconceived theory or hypothesis. Two research team members collaboratively simultaneously reviewed identical data segments and independently documented their observations. Throughout this phase, we curated recurring {\textit{themes}} that arose in the analysts' perceptions and expectations of authoring experiences with AI-assisted tools (e.g. trust, efficiency, and interaction). Subsequently, we conducted a comprehensive coding of the interview transcripts, to systematically identify these themes. This process involved an iterative development and modification of codes as research team members worked their way through the collection of transcripts. To maintain the rigor and precision of our coding process, two coders periodically conducted cross-checks.}

\subsection{Key Findings}
\label{sec:formative_findings}
\subsubsection{\textbf{KF1.} Viewing technology as a means to enhance human capability.}
While examining intelligence analysts' views on advanced technology, an overwhelming majority (9 out of 10) emphasized the crucial role of digital technologies and artificial intelligence in enhancing their capabilities, specifically in generating situation reports. These tools are regarded not as mere process accelerators, but as essential elements that enrich their work by improving research efficiency, idea generation, and clarity of information. This perspective contrasts with the simplistic media depiction of these technologies as mere replacements for human effort. Instead, analysts view them as valuable enhancements to their workflow, particularly in high-pressure or resource-limited scenarios. For instance, one analyst commented:

%When exploring the intelligence analysts' perspectives on advanced technology, 9 out of 10 participants (IA1-IA7 \& IA9-10), described the vital role of digital technologies and AI in augmenting their capabilities, particularly in the context of situation report generation. These technologies were not seen merely as separate tools for speeding up processes, but as key contributors integral to enriching the analysts' work, by improving aspects like research efficiency, brainstorming, and clarity of information. Contrary to the often simplistic portrayal of these technologies in popular media as mere substitutes for human effort, analysts perceived them as providing valuable enhancements to their workflow, especially under high-pressure situations or resource constraints. For instance, one analyst commented:} %\heng{what was the negative comment from the person who disagree?}

\begin{quote}
``There's so many parts of authoring a situation report, each requiring strict and robust procedures. I wish I could have an AI partner to help me. It could make me better at my job.'' (IA6)
\end{quote}

This highlights a paradigm shift in the perception of technology within intelligence work, where it is seen not as a substitute, but as a vital complement that amplifies human skills.

%This insight underscores a paradigm difference in how technology is viewed in intelligence work – not as a replacement for human skills, but as a powerful ally that complements and strengthens human capabilities.}

\subsubsection{\textbf{KF2.} Trusting and relying on machines, as with humans.} The majority of participants (8 out of 10) exhibited a tendency to attribute human-like qualities of trust and reliability to AI systems, akin to their assessment of human colleagues. Analysts recognized AI as a dependable information source, comparable to a human co-worker, with a focus on its consistent delivery of high-quality outputs. The criteria for trusting AI closely resembled those for human interactions: the ability to provide dependable information, transparency in reasoning, and a foundation in verifiable facts. One participant articulated this equivalence in trust establishment:

%Most participants (8 out of 10) conveyed a tendency to attribute human-like qualities of trust and reliability to AI systems, paralleling the way they evaluate their human counterparts. Analysts designated AI as a reliable source of information, similar to a human colleague, with an emphasis on the AI's ability to consistently deliver quality outputs. The criteria for trust in AI, therefore, mirrored those applied to human interactions: the ability to provide dependable information, transparency in the process of deriving conclusions, and a foundation in verifiable facts. When inquired about how and why they would trust AI and human and the similarity in response, an intelligence analyst pointed out:} 

\begin{quote}
``After comparing my expectations between a human and an AI colleague, I can't say there's much of a difference. Trust is built the same way regardless of who it's towards. Just as I would trust a colleague that can explain their work, I could trust an AI that could show its workings.'' (IA1) 
\end{quote}

Interestingly, analysts did not set higher standards for AI than for human colleagues. This parity in trust and reliability criteria suggests that participants viewed AI as an equal collaborative partner, assessing its competence and trustworthiness on the same grounds as a human team member.

%Curiously, the analysts did not impose additional requirements or expectations on AI systems beyond what they would expect from a human colleague. The equivalence in the standards of trust and reliability, as expressed by participants, indicated that they viewed AI as a collaborative partner and judged its competency and trustworthiness by the same standards and merits as those of a human team member.}

\subsubsection{\textbf{KF3.} Training and guiding AI} 
Our research identified a split in intelligence analysts' perspectives on their role in training and guiding AI systems. Four out of ten participants advocated for substantial control over AI, emphasizing the need for an interactive system that allows them to influence everything from information source selection to narrative shaping in reports. They prioritized the ability to refine AI outputs based on their expert judgment. Two participants stated:

%We found a split in intelligence analysts' attitude to their involvement in training and guiding AI systems. 4 out of 10 participants expressed a strong desire for high-level control over AI systems. This group emphasized the need for a highly interactive system where they could exert significant influence, from selecting information sources to tailoring the narrative in reports. They believed in defining the quality of AI outputs based on their expert judgment, desiring systems that allowed for extensive fine-tuning. Two analysts stated:} 

\begin{quote}
``We're trained to be great at what we do. Isn't AI, like picking a random university student, and asking them to do our job?'' (IA2)
\end{quote}

\begin{quote}
''It's not about control. If someone is going to help me, I'm going to make sure they do it right.'' (IA7)
\end{quote}

In contrast, the majority (six out of ten) favored a more hands-off approach, highlighting that situation report creation follows well-established, standardized procedures suitable for AI implementation. They perceived AI involvement as an extension of routine oversight, akin to reviewing a junior colleague's work:

%Conversely, the remaining six participants viewed the role of AI differently. They pointed out that the process of creating situation reports is well-documented and follows strict, standardized procedures. According to them, these procedures are areas where AI could excel, as these standards and protocols could be effectively distilled into AI systems to produce concise and accurate reports. While acknowledging the need for oversight and occasional fine-tuning, they saw this as a routine aspect of their work, not unique to AI.} 
\begin{quote}
''There's a specific way we have to do each action, and making reports is no different. I just need to tweak small details as I would when reviewing other junior ranking officer's work.'' (IA10)
\end{quote}

This variance in attitudes seems to highlight a broader debate within intelligence work: the balance between human expertise and automated efficiency.

%This split in attitude and perceptions among intelligence analysts regarding the degree of human involvement and control desirable in AI-assisted processes also reflects a broader debate about the balance between human expertise and automated efficiency in intelligence work.}

==> sections/4_Collaborative_Design.tex <==
\section{Collaborative Design}
\label{sec:collaborative_design}

%\heng{Echo Revanth's comments - it's important to align section 5's components back with these design principles, e.g., how do the innovative components such as question generation and claim detection align with these principles? You can also point to section 5's subsections here in section 4.}

To gain a better understanding of the composition process of situation reports, we expanded the design opportunities identified in the formative study with subsequent collaborative design (CD) sessions with 10 participants (IA1-IA10). The goal was to capture tangible design strategies and recommendations from users about how they, as intelligence analysts, navigate, research, and author their situation reports.

\subsection{Process}
\subsubsection{Participants}
To enable us to build on the insights and findings of the formative study, the original participants (IA1-IA10) were sustained in the collaborative design phase.

\subsubsection{Procedure}
Each study session consisted of three distinct components: a Workflow Review using Storyboards, a hands-on Training Task, and a Simulation Report exercise. These sessions, conducted virtually, spanned approximately one hour each, with participants receiving compensation consistent with the rates in our formative study. 

%\heng{Did you also ask them to compare with gpt+bing? maybe good to add for camera-ready}

\begin{enumerate}
    \item \textbf{Workflow Review with Storyboards}
    \begin{enumerate}
        \item \textbf{Introduction to Storyboards:} In our study, participants engaged with a low-fidelity storyboard (shown in Figure \ref{fig:storyboard}), where each panel depicted a distinct phase in situation report creation. The storyboard, designed based on insights from our formative study, aimed to establish a comprehensive understanding of the workflow for generating situation reports. The construction of the storyboard was guided by detailed information on situation reports (in \S{\ref{sec:situation_report_background}}), whereas the key findings (in \S{\ref{sec:formative_findings}}) shaped the formulation of probing questions presented during participant interaction with the storyboard.
        \item \textbf{Annotation and Brainstorming:} Participants were tasked with providing detailed descriptions of each storyboard panel to ensure comprehension of the depicted scenario and workflow. Additionally, they annotated the storyboards for subsequent analysis, establishing a basis for identifying user needs and interaction strategies. This phase also included a semi-structured interview, with questions derived from the key findings of the formative study. (e.g. KF1: In which of these steps, would you be willing to use technology? How and why would you use it?) 
        \end{enumerate}
    \item \textbf{Training Task}
    \begin{enumerate}
        \item \textbf{Familiarization Exercise:} Participants simulated each storyboard step using sample situations to gain practical workflow experience. Two distinct question sets, varying in scope and complexity, were assigned to IA1-IA5 and IA6-IA10.          
        \item \textbf{Tool Utilization:} Candidates were advised to utilize diverse resources, including web searches like Google and Bing, and Large Language Models such as ChatGPT, for task completion.     
        \end{enumerate}
    \item \textbf{Simulation Report}
    \begin{enumerate}
        \item  \textbf{Situation Handling:} Participants were each presented with a unique situation and tasked (as above, in the training task) with facilitating the end-to-end process of creating a complete situation report.
        \item \textbf{Process Documentation and Ideation:} Throughout this simulation, participants documented their rationale for tool selection, challenges encountered, and potential system improvements. This feedback was critical to defining the Design Strategies (in \S{\ref{sec:design_strategies}}).
    \end{enumerate}
\end{enumerate}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{tables/storyboard.jpg}
    %\vspace{-1em}
    \caption{Storyboard used in the collaborative design sessions with intelligence analysts.}
    \label{fig:storyboard}
\end{figure}

\subsection{Results}
\label{sec:collaborative_results}
In analyzing the data collected during the collaborative design sessions, we found three clear themes emerged.

\label{sec:formative_results}
\subsubsection{Enhancing analytical efficiency and reducing cognitive load} 
\label{sec:4_2_1}
Participants expressed a need for user interfaces that closely mirror their mental models of data analysis and report generation. Specifically, one analyst described their ideal tool as, ``A system that reflects our thought processes, almost as if the tool 'thinks' like an analyst.'' (IA1). Such feedback indicates a preference for interfaces that are instinctive and reduce the need for deliberate navigation, thereby enabling analysts to concentrate on the strategic aspects of their work. Moreover, analysts (IA1-IA5, IA7) underscored the significance of customizing data presentation in the interface to efficiently distill valuable insights from raw data, thereby decreasing the time and effort needed for data analysis.

\subsubsection{Trust and reliability in AI-systems} 
\label{sec:4_2_2}
Here the focus was on building trust in how the system operates, through its interpretability and transparency. Participants stressed the importance of understanding the automated system's underlying logic and methodology. Analysts called for explicit clarity in the system's data processing and analysis methods. Specifically, one analyst stated, ``For me to trust the system, I need to understand how and what it does. I want to know the brains behind it.'' (IA3). 

Transparency in data sources and information flow was another key aspect highlighted by the participants, emphasizing the importance of traceability from report contents to original sources. This traceability enhances the credibility and trustworthiness of the automated system. As IA9 noted, "Understanding where the information is coming from is so so important. It's knowing that the information didn't just come from nowhere." (IA9).

The sessions indicated a marked preference for outputs that enhance user comprehension and verification of the system's conclusions. Analysts favored reports offering summaries with annotations or data source references, allowing them to corroborate the system's findings against their own expertise. This method promotes an interplay between building trust with personal verification. One participant emphasized the need for transparency, requesting, ``Explain to me how you came up with the answer.'' (IA2). 

\subsubsection{Customization and flexibility with automated tools.}
\label{sec:4_2_3}
Participants desired a tool that not only accommodates different analytical styles but also various levels of detail and complexity in reporting. One analyst (IA1) highlighted the necessity for an interface that can dynamically alternate between in-depth data analysis and high-level overviews, depending on the intended reason. Additionally, there was a notable interest in a platform that allows users to specify the sources of data, such as news reports, social media feeds, and official records. This would enable the aggregation and analysis of information from these diverse origins in a unified manner, providing a more comprehensive perspective on the subject matter.

\subsection{Design Strategies}
\label{sec:design_strategies}
From the findings of the formative study (in \S{\ref{sec:formative_study}}) and the results of the collaborative design above, we identified the following design strategies:

\begin{itemize}
    \item \textbf{DS1:} Given the emphasis on reducing cognitive load and enhancing analytical efficiency (KF1 and \S{\ref{sec:4_2_1}}), the system will be designed with an interface, that mirrors intelligence analysts' natural processes of data analysis and report generation.
    \item \textbf{DS2:} To increase efficiency (\S{\ref{sec:4_2_1}}), the system will integrate features to automate time-intensive tasks such as question curation and preliminary research, thereby reducing analysts' manual workload and enabling greater focus on strategic analysis and decision-making.
    \item \textbf{DS3:} The design, addressing the need for trust and reliability (KF2 and \S{\ref{sec:4_2_2}}), will convey clear explanations of the system’s data processing algorithms and criteria. This includes transparent data sourcing, providing references within reports, and tools for users to easily understand and verify the system's conclusions. The design will also facilitate incremental trust-building through consistent and validated performance over time.
    \item \textbf{DS4:} Addressing the themes of customization and flexibility (KF3 and \S{\ref{sec:4_2_3}}), the system will offer a high degree of adaptability to accommodate various analytical styles and levels of detail in reporting. It will include features for adjusting the depth of analysis, focusing on specific data sets, and seamlessly integrating various data sources.
    %\item \textbf{DS5:} \textcolor{blue}{The system will be equipped with transparent mechanisms that elucidate the processes of data handling and summary creation (\S{\ref{sec:4_2_1}}). By making these processes clear and understandable, the design aims to deepen user comprehension of the automated functions, thus enhancing confidence and trust in the system's outputs.}
\end{itemize}










==> sections/5_SmartBook.tex <==
% \section{Problem formulation}
\section{SmartBook System}\label{sec:smartbook}

\begin{figure}[t]
% \def\w{0.55\linewidth}
\centering
% \begin{tabular}{*3c}
% \includegraphics[height=\w, trim=35 30 35 10]{Web.pdf}
\includegraphics[width=1\linewidth]{tables/smartbook.jpg}
% \end{tabular}
\caption{A screengrab of SmartBook's front-end interface. Within the given situation, the user can navigate timelines (F1), explore strategic questions related to an event (F2), read the overarching summary on a given strategic question (F3), control the depth and length of information (F4), investigate all the claims in the summary (F5), correlate each claim to corresponding summary fragment (F6), investigate the source metadata (F7) and read the context in which the claims were extracted (F8).}
\label{fig:system1}
\end{figure}
%\subsection{Framework}
%\revanth{Notes: This section has been considerably compressed, with details moved into the appendix as per reviewer suggestions.}
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/SmartBook_arch2.png}
    \vspace{-0.5em}
    \caption{\small Overall workflow for constructing \textit{SmartBook}. Given the articles corresponding to a specific timeline, the figure shows the process for obtaining the chapters, their section headings, and the corresponding section content.}
    \label{fig:overall_workflow}
    \vspace{-1em}
\end{figure}

Using the four design strategies, we developed \textit{SmartBook}, an AI-assisted system for situation report generation that provides analysts with a first-draft report to work from as they respond to time-critical information requirements on emerging events.

SmartBook consists of: 1) An intuitive user interface (shown in Figure \ref{fig:system1}) built using the design strategies from \S{\ref{sec:design_strategies}}, and 2) a back-end framework (shown in Figure \ref{fig:overall_workflow}) that, when given a collection of documents from a variety of news sources, automatically generates a situation report. The situation reports, as per analysts' expectations and recommendations, are presented with a logical structure and organized chronologically as timelines, while being grounded to factual content.

%Given a collection of documents from a variety of sources, we aim to generate a situation report that embodies characteristics such as containing salient information that is presented with a logical structure and organized chronologically as timelines, while being grounded to factual content.} 

In this section, we describe the various components within SmartBook, along with emphasizing the advantages of each aspect of SmartBook's design for users (i.e., intelligence analysts) and for recipients of the final SmartBook report (i.e., decision-makers) who both initiate information requirements and are downstream readers. For in-depth technical details on SmartBook's back-end functionality, we point the reader to Section \ref{sec:appendix} of the Appendix. 
 
%\textcolor{blue}{Figure \ref{fig:overall_workflow} gives an overall workflow diagram for our approach, with each of the steps briefly described below. 
%Further,  

\begin{enumerate}
    \item \textbf{Major Events within Timelines as Chapters}: Situation reports cover event progressions over considerably long periods. Hence, it is beneficial to organize such reports in the form of timelines (F1 in Fig. \ref{fig:system1}) informed by DS1, which enables seamless report updates~\cite{ma2023structured} with new events and helps facilitate~\cite{singh2016expedition} users tracking and understanding of situation context. Timelines aid intelligence analysts in understanding event progression and predicting future trends by organizing events chronologically and highlighting cause-and-effect relationships. For readers, especially those less familiar with the subject, timelines provide a visual guide to easily grasp the sequence and significance of events in a scenario.    
    Our automatic situation report has timelines to provide a coherent, chronological representation of event developments (DS1, DS2). Each timeline spans a duration of N weeks\footnote{While more fine-grained timelines can be considered for relatively short-term events, we consider $N=2$ for a more spread-out scenario such as the Ukraine-Russia crisis. This reflects similar biweekly reporting timelines considered by organizations such as \href{https://datafriendlyspace.org/reports/}{Data Friendly Space}.}. %, allowing for manageable capturing and focused analysis of significant newsworthy occurrences. 
    The newsworthy major events within a timeline are identified via clustering~\cite{jain1988algorithms} news articles, to serve as the foundation for corresponding chapters within SmartBook. A key to further improving interpretability is deriving a short chapter name for the event, which we achieve by generating a short headline using multi-document summarization~\cite{headline2020}. %to facilitate information readability and retrieval for the timeline within the situation report. 
    Moreover, with the generated chapter name, we query Google News to obtain an expanded set of news articles relevant to the event.\\    
    
    \item \textbf{Strategic Questions as Section Headings}: Guided by DS2, a situation report should be logically structured with descriptive chapter headings and section titles for ease of understanding and information access.
    (F2 in Fig. \ref{fig:system1}). Structured reports benefit intelligence analysts by simplifying complex situation analysis, offering easy navigation, clear information hierarchy, and improved context understanding. For less experienced readers or those seeking specific information, the logical structure enhances information retrieval, and comprehension, while providing an intuitive mental map, making reports more reader-friendly.     
    Beyond simply describing event details in each major event chapter, SmartBook aims to provide information from a strategic perspective that can help aid decision-making and policy planning. To guide such detailed chapter analysis, we incorporate a logical structure through automatically generating section headings in the form of strategic questions relating to each major event. These question cover detail such as the possible motivations of the actors in an event and the future implications of the event. The questions are generated by prompting LLMs~\cite{brown2020language} with a grounded context in the form of news articles from the event cluster. Further, we promote diversity in the questions by using sampling strategies~\cite{holtzman2019curious} during generation, and then automatically de-duplicate~\cite{Chen2017QuoraQP} to obtain a set of unique strategic questions about the event. 
    
    \item \textbf{Extraction of Claims and Hypotheses:} 
    Automated situation report generation should be able to identify and extract the most scenario-relevant and crucial information across multiple documents (F5 in Fig. \ref{fig:system1}). Intelligence analysts, given high stakes nature of their work, but their limited time, need systems that quickly identify key information in documents (DS2). This enables them to focus on urgent matters without sorting through irrelevant data. Readers of the situation report benefit from information salience because they are presented with a concise, relevant overview of a situation. Essential points are highlighted, enhancing accessibility and clarity of the report's implications. Moreover, we present the bias of each news source\footnote{We collect information from \href{https://www.allsides.com/media-bias/ratings}{AllSides Media Bias} ratings.}, to help analysts consider information presented from different perspectives.
    Providing readers with a comprehensive understanding of event context requires foraging for different claims and hypotheses from the source documents (i.e., news articles) that help explain a situation \cite{toniolo2023human}. We adopt a Question Answering (QA) formulation to identify claims relevant to a given strategic question, motivated by recent studies \cite{reddy2022newsclaims, reddy2022zero} which have shown that directed queries can automatically extract claims from news articles relevant to a specific topic.\\
        
    \item \textbf{Grounded Summaries as Section Content}: 
    To be reliable, a situation report must be grounded in verifiable sources, as grounded factual content helps to build credibility (DS3). Reliable information is crucial for analysts, enabling them to verify facts from sources and draw solid, evidence-based conclusions. This reduces the need for additional fact-checking, as evidence is directly linked. Moreover, for those readers wanting to delve deeper or explore related topics, the embedded links act as a springboard to more extensive research (F6, F7, F8 in Fig. \ref{fig:system1}). Further, we present summaries with three levels of detail (less detailed, normal and more detailed corresponding to 2-3 sentences, 4-6 sentences and 2 paragraphs respectively) (F4) to allow readers to customize the level of detail at which they prefer to consume content, building from DS4.
    The individual sections comprise the core content of our situation report, and contain grounded, query-focused summaries which address the strategic questions. The extracted claims are combined into a concise summary by using LLMs with a novel prompting mechanism, which also generates citations linking each summary fragment to its factual input claim. This allows analysts to verify the summary information against input sources as needed.
\end{enumerate}
%
Ultimately, the structured incorporation of timeline chunking, major event chapter clustering, strategic question headings, claim extraction and query-focused section summaries within chapters enables our SmartBook system to generate reliable, insightful reports to assist analysts in responding to information requirements about time-sensitive, emerging situations. 





==> sections/6_System_Evaluation_Overview.tex <==
 \section{System Evaluation Overview}
To comprehensively evaluate SmartBook and its efficacy in aiding intelligence analysis, our approach encompassed two distinct but interrelated studies: a user study and a content review. The user study (in (\S{\ref{sec:usability_study}}) aimed to answer four research questions concerning SmartBook's usability, focusing on its effectiveness for intelligence analysts and decision-makers in generating and interacting with situation reports. Complementing this, the content review (in \S{\ref{sec:content_review_study}})  assessed the quality of SmartBook's summaries, focusing on readability, coherence, and relevance, alongside an editing study where an expert analyst edited the generated reports to understand their utility as preliminary utility. These combined efforts provided a holistic understanding of SmartBook's practicality and effectiveness in the field of intelligence analysis, offering insights into both its user experience and content quality.

%{\textcolor{red}{\textbf{is this Section 6 going to remain this way, as a standalone section to overview the next 2 sections? -- Clare}}}
%\revanth{Yep, that's the plan. Does this seem like an outlier?}

==> sections/7_User_Study.tex <==
\section{User Study: Evaluating the System}
\label{sec:usability_study}
During the user study, we conducted an interview with semi-structured questions and a post-study questionnaire on the usability of the SmartBook. The study investigated the following research questions:
%\revanth{RQ3 seems abrupt. Maybe move it to last RQ and also brief mention earlier that this was done from the perspective of both intelligence analyst (user) and decision-makers (downstream reader)}
\begin{itemize}
    \item \textbf{RQ1:} Can intelligence analysts successfully use SmartBook to generate situation reports?
    \item \textbf{RQ2:} How do intelligence analysts interact and leverage the features within SmartBook?
    \item \textbf{RQ3:} Do intelligence analysts find SmartBook intuitive, usable, trustable and useful?
    \item \textbf{RQ4:} How do decision-makers interact, perceive and use SmartBook?
\end{itemize}

\subsection{Method}

%\heng{a lot of these content overlaps with those in section 3, is this intentional?}
%\daniel{Thematically, there will be content overlaps with the previous sections. However, this is a reaffirmation that we developed SmartBook in line with user expectations and needs. I've added more details, to be granular about the findings in the user study.}

\subsubsection{Recruitment}
For this user study, we recruited a total of 12 participants, comprising of 10 intelligence analysts (IA1-IA10) and 2 decision-makers (DM1 and DM2). The recruitment process for the intelligence analysts involved maintaining the existing cohort from the formative study and collaborative design. Each analyst was compensated at the same rate as previous studies. 

We implemented a targeted outreach strategy to recruit decision-makers for our study. These participants, identified through email addresses sourced from government boards and social media profiles (e.g., LinkedIn, Twitter), were self-identified professionals who make decisions based on prepared reports in their official capacity. Our group comprised of individuals with current or past experience on Canadian government boards. These decision-makers engaged in the initial qualitative study but did not partake in the subsequent post-study questionnaire, due to time constraints. Unlike intelligence analysts, these participants did not receive compensation due to their government affiliation.

%\textcolor{blue}{For the decision makers, we employed a targeted outreach strategy. We reached out to potential participants utilizing emails obtained from government boards or social media platforms (e.g. LinkedIn, Twitter). The candidates self-identified as decision makers, defined as individuals who have made decisions based on reports which had been prepared for them in their professional capacity. The decision makers recruited for our study included individuals who are currently or have previously served on government boards in Canada. The decision makers participated in the qualitative study described first below, but not the post-study interview due to their limited availability. Unlike the intelligence analysts, the decision makers were not compensated due to their government affiliation.} 

\subsubsection{Study Task}
Each user study session was structured into four segments: (i)~an introductory overview, (ii)~a free-form investigation, (iii)~a guided exploration, and (iv)~a concluding reflective discussion. These sessions, each lasting about an hour, were remotely conducted, with participants engaging through their personal computers and browsers, and screen sharing their activity.

Upon commencement of the study~(i), participants received a concise introduction to SmartBook, outlining its core premise. This orientation was designed to acquaint them with the system without biasing their exploration. Subsequently~(ii), participants were invited to freely investigate SmartBook, with the specific task of exploring a minimum of three questions across five chapters of their choosing. This approach afforded substantial freedom, enabling interactions with the user interface that reflected their natural inclinations and interests.

Following the free-form investigation, participants were systematically introduced to the SmartBook framework. This process entailed tracing the journey from a chosen question related to a specific event within a designated timeframe, to the corresponding claims, contexts, and sources, culminating in a summarized answer. This tracing aligned with the F-numbered features illustrated in Figure~\ref{fig:system1}. The selection of questions for this exercise were informed by criteria such as question complexity and the variety of sources referenced. During this guided exploration phase~(iii), we ensured comprehensive exposure to each SmartBook feature, aiming for participants to fully grasp the system's capabilities.
Subsequently, a semi-structured interview~(iv) was conducted to gather reflective feedback on the participants' experience with SmartBook, focusing on its efficacy and potential areas of enhancement.

Finally, to conclude the session, participants were asked to complete a post-study questionnaire. This questionnaire was focused on assessing the usability of SmartBook, gathering quantitative data to complement the qualitative insights gained from the semi-structured interviews. Decision-makers were exempted from the post-study questionnaire.

\subsection{Results}
The data collection and analysis followed a similar method as in \S{\ref{sec:formative_analysis}}, with the addition of a post-study questionnaire. Upon collecting, discussing and iterating on the data, behaviors and insights were merged into the following themes:

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{tables/userstudy.jpg}
    \vspace{-3em}
    \caption{Quantitative results from the post-study questionnaire in the user study.}
    \label{fig:userstudy}
\end{figure}

%\revanth{Write a brief outline here on how you came up with or grouped these themes together.}
%\revanth{Add in a reference to and discuss the quantitative results shown in Figure 5.}
%\revanth{For subsection, we should add in a relevant quote or two from what the analysts/decision makers said in the studies/interviews.}

\subsubsection{UI Understandability and Interaction}

%The user interface (UI) of SmartBook was highly effective, as evidenced by the ease of navigation and feature discovery demonstrated in our data analysis. All participants (10 out of 10) successfully discovered each feature in SmartBook, as seen in (ii), demonstrating the UI's ease-of-understanding and low learning curve. Participants (IA2, IA3, and IA6) notably appreciated the logical organization into chapters and questions, clear navigation, and easy access to various system components. The high feature discovery rate indicates the UI's alignment with users' cognitive processes during information gathering, allowing intuitive interaction and access to system capabilities with minimal training. This positively addresses {\textbf{RQ1}}. IA2 particularly noted the advantages of SmartBook's similarity to their manual process of creating situation reports.:

The structured layout of the user interface (UI) was notably effective, as seen in the free-form investigation~(ii) with a 100\% feature discovery rate (10 out of 10 participants). All participants successfully engaged with key features, underscoring the UI's design intuitiveness. Participants IA2, IA3, and IA6 commended the logical organization into chapters and questions, as well as the straightforward navigation and component access. This high feature discovery rate indicates that the UI aligns with users' cognitive patterns, facilitating intuitive interaction without extensive training, providing us with a positive response to {\textbf{RQ1}}. Participant IA2 appreciated the UI's alignment with their existing workflow:

%The structured layout of the user interface (UI) stood out in the data analyses for the ease with which participants freely navigated and discovered the features in SmartBook, as seen in the free-form investigation~(ii) with a 100\% task completion success rate (10 out of 10 participants).Each participant successfully discovered and utilized key features of the system, a testament to the UI's design effectiveness. Participants (IA2, IA3, and IA6) highlighted the logical breakout of information into chapters and questions, the readily accessible and clear navigation from the summary to each relevant claims, and the ease with which they could access different system components. The high feature discovery rate also suggests that the UI aligns well with users' cognitive organization of content collected during their information foraging. This enables them to intuitively understand how to interact with the system and access its capabilities without extensive training or guidance, providing us with a positive answer to {\textbf{RQ1}}. IA2 mentioned the benefits of the SmartBook mirroring their manual process of generating situation reports: 

\begin{quote}
``I appreciate how I don't have to learn a new workflow just for a tool. It works how I would work.'' (IA2)
\end{quote}

This sentiment was further emphasized in the post-study questionnaire. As seen in the results in Figure~\ref{fig:userstudy}, 70\% of participants strongly agreed that most intelligence analysts would learn to use the system very quickly, while 80\% strongly disagreed that the system was difficult to navigate and use.
%This sentiment was further emphasized in the post-study questionnaire (\ref{sec:usability_study}, where 7 and 3 participants, respectively, strongly agreed and agreed that they believed most intelligence analysts would learn to use the system very quickly. This was also consistent with the responses from 8 and 3 participants, respectively, who strongly disagreed and disagreed that they found the system difficult to navigate and use. 
However, responses to issues raised by \textbf{KF3} and \textbf{DS4} revealed mixed views on UI flexibility, specifically in personalization and customization. While most found the tool easily integrateable into their workflow, a minority (30\%) remained neutral. When further prompted, participants IA8 and IA9 described the UI as a ``one size fits all'' solution, lacking personalization. As per \textbf{RQ2}, IA9 further highlighted that although it is a streamlined experience, it is inflexible to differing priorities:

%However, the participants' responses provided us with mixed answers to issues raised by {\textbf{KF3}} and {\textbf{DS4}} concerning the flexibility of the design (personalization and customization).  While most participants agreed that the tool could easily be integrated into a situation report generation workflow, some participants (3 out of 10) were neutral on its integration. When further prompted, they (IA8 and IA9) stated while the tools was generalizable and adaptable, it was nonetheless a "one size fits all" solution, that they couldn't personalize to their own experiences. An analyst further highlighted that although it is a streamlined experience, it is inflexible to differing priorities, per {\textbf{RQ2}}: 

\begin{quote}
``I don't deny that this tool is easy to use and quite understandable. But, for me to use some parts like finding sources that back a question, I have to interact with every part of the tool before I get there.''
\end{quote}

\subsubsection{Trust and Severity of Impact}
In the study, trust in the SmartBook system developed progressively, resembling the formation of trust in a human analyst. Initially, users exhibited skepticism, thoroughly scrutinizing the system's sources and assertions. This included validating the authenticity of sources, the accuracy and pertinence of ratings, and the correct representation of context. As users became more acquainted with SmartBook and evaluated its reliability, their dependence on extensive source verification lessened. As can be seen in Figure \ref{fig:userstudy}, three out of ten participants did not feel the need to conduct additional research beyond the presented information to trust the tool, while another three felt additional research was necessary. The necessity of further research was linked to the context of use; as one analyst stated:
%Trust formation with SmartBook emerged gradually during the study, akin to building a relationship with a human analyst. Initially, users approached the system with a degree of skepticism, meticulously verifying the sources and claims presented. This rigorous validation process involved checking the authenticity of each source, assessing the accuracy and relevance of the ratings, and ensuring the context was correctly captured. Over time, as users familiarized themselves with SmartBook's structures and assessed its content for reliability, their reliance on intensive source verification decreased. Three out of ten (\ref{sec:usability_study} participants disagreed that they found it necessary to research the information beyond what was presented in order to trust the tool, while 3 out of 10 participants either agreed or strongly agreed that they did find it necessary to do further research. However, when probed specifically on why they found this necessary, an analyst explained: 

\begin{quote}
``It's more about what situation we're in. If we provide incorrect information, people can get hurt.'' (IA3)
\end{quote}

This trust was found to be context-dependent, aligning with the concerns in \textbf{KF2} and \textbf{DS3}. Participants IA1 and IA2 noted that their trust varied based on the ``impact severity'' or the potential negative consequences of disseminating incorrect information. Nonetheless, a majority (eight out of ten) concurred that the information provided was accurate and reliable, a positive answer to {\textbf{RQ3}}. Upon probing, IA3 contrasted this with traditional military intelligence, which is often unquestioned.

%Put another way, the users' trust in the system was deemed context-sensitive, harkening back to issues raised in {\textbf{KF2}} and {\textbf{DS3}}. Participants (IA1 and IA2) suggested that their willingness to trust the system's output, depended on "impact severity", i.e., the negative consequences to providing incorrect information in their situation report to the downstream reader. However, in contrast to the previous statement, 8 out of 10 participants agreed that the information provided by the report was accurate and reliable, a positive answer to {\textbf{RQ3}}. Due to IA3's feedback on the prior question, we requested further elaboration: 
\begin{quote}
``Traditional intel within the military is a black box. You're given information, and you're told to blindly trust, rely and not question it. If we're talking about the accuracy and reliability of information, SmartBook at least reassures me of where it all came from, and shows me I could grow to trust it.'' (IA3)
\end{quote}

\subsubsection{Perceived Benefits for Intelligence Analysts}
The primary benefit identified was the substantial reduction in time and effort required for compiling and analyzing complex data. SmartBook's automation of initial report generation processes, such as data collection and summarization, was highly valued by analysts as it allowed more focus on thorough analysis and strategic planning. As seen in Figure \ref{fig:userstudy}, all participants agreed on the tool's utility in assisting intelligence analysts in creating situation reports, expressing satisfaction with the system-generated reports, supporting a positive response to \textbf{RQ1}.

%The most significant perceived benefit was the expected, dramatic reduction in time and effort otherwise required to compile and analyze complex data sets. Analysts appreciated how SmartBook automated the initial stages of report generation, such as data collection and summarization, allowing them to dedicate more time to in-depth analysis and strategic thinking. All 10 participants agreed to a degree (\ref{sec:usability_study}, that the tool could be useful for intelligence analysts to create situation reports and were satisfied with the report generated by the system, providing us with another positive response to {\textbf{RQ1}}. 

Regarding the necessity of significant edits to the system-generated reports, participants IA5-IA9 suggested that this need was not inherently due to report deficiencies but varied based on the report's intended purpose or audience. We later conduct a study, described later in \S{\ref{sec:editing_study}}), to understand the extent of edits needed.

%When prompted with their varying perspectives on whether it was necessary to make major edits to the system-generated situation reports, participants (IA5-IA9) noted this wasn't due to deficiencies within the reports per se, rather this would be dependent on the "intended purpose or audience". To investigate the objective basis for these varying claims about the need to edit, we also completed an editing study (Section 8.3).

%\revanth{Needs a bit of expansion and tt reads too generic currently. IMO we can't claim we did study with decision makers without giving thorough/specific details. Might need to add one more point here.}
\subsubsection{SmartBook as a Learning Tool for Decision-Makers}
Decision-makers highly valued SmartBook's ability to rapidly deliver accurate and easily digestible information. Their primary engagement with the interface centered around utilizing the summaries, to learn about different topics in various degrees. The system's effectiveness in simplifying complex data into structured, clear formats was particularly appreciated, to help aid in swift understanding and decision-making processes.
%For decision makers, the capability of SmartBook to provide rapid, accurate, and easily digestible information was considered invaluable. Rather than exploring different components of the SmartBook interface, they focused in on the summaries, learning about different topics in various degrees. They particularly valued the system's capacity to distill complex data into concise, structured formats that would facilitate their own quick understanding and decision-making. One of the decision makers remarked:

\begin{quote}
''When something happens, I'm expected to know about it. I want to learn as fast as I can, and get the information I only need.'' (DM2)
\end{quote}

Although data lineage and source transparency were recognized as important, these were considered secondary to the primary need for timely and format-specific information delivery. While SmartBook's target users are intelligence analysts, the decision-makers' view highlights SmartBook's dual functionality as both an analytical tool and a decision-support system, providing a key capability for the high-paced and information-intensive needs of decision-makers, addressing \textbf{RQ4}.

%While aspects like data lineage and source transparency were important, these were considered secondary to the primary need for timely and format-specific information delivery. While SmartBook's target users are intelligence analysts, the decision makers' view highlights SmartBook's dual functionality as both an analytical tool and a decision-support system, providing a key capability for the high-paced and information-intensive needs of decision makers, addressing {\textbf{RQ4}}.



==> sections/8_Content_Review.tex <==


\section{Content Review: Evaluating the Generated Content}
\label{sec:content_review_study}

%\heng{It will be more exciting to add the examples comparing with gpt+bing, including pages 9-14, 81-82 and in this set of slides: https://blender.cs.illinois.edu/ALTA\_NLP\_SmartBook\_HengJi.pdf}


In this section, we seek to evaluate the quality of the text summaries generated by \textsc{SmartBook}. Our approach is complementary to the usability study in \S{\ref{sec:usability_study}}, which assessed whether \textsc{SmartBook} is useful to intelligence analysts and decision-makers. We first evaluate the system's summaries for readability, based on coherence, relevance, and tactical usefulness of the information (in \S{\ref{sec:readability_study}}). Next, we evaluate whether the automatically generated situation reports can serve as a useful preliminary draft with an editing study to ascertain how extensively an expert analyst edits the summaries to deem them acceptable (in \S{\ref{sec:editing_study}}).

%To do so, an evaluation schema was developed by the expert intelligence analyst, based on coherence, relevance and tactical usefulness of the information. 
\subsection{Participant Recruitment}
%\revanth{Should we be calling the students as text evaluators or text annotators or text analysts?}
The studies involved two participant groups: one senior expert analyst (SA1) and six text evaluators (TE1-TE10). 
The expert, affiliated with a US national defense and security firm, possessed a decade of experience in intelligence analysis, training, and AI-based tool assessment. This included researching intelligence tutoring systems and testing AI-based search tools for analysts. The text evaluators, all fluent in English and US-based, held Computer Science degrees ranging from Bachelor's to PhDs, and had prior text annotation experience. There were three natural language processing graduate students and three undergraduates in computer science. The participants reflected the composition of a training unit, with the senior expert providing supervision and training in system evaluation. Compensation varied between groups, with the expert working under a research contract and evaluators receiving \$20 per hour.
%Two types of participants were recruited: (1) an expert analyst and (2) 6 text evaluators. The expert analyst, sourced through a partnership with an independent US-based national defense and security firm, had 10 years of experience collaborating with intelligence analysts, particularly in the realms of training and tool evaluation. This included researching intelligence tutoring systems and testing AI-based search tools with for analysts. The six text evaluators had advanced degrees in Computer Science (ranging from Bachelors to PhDs) and prior experience in text annotation. They included three natural language processing graduate students and three computer science undergraduates, all fluent in English and based in the US. The recruitment of a single expert analyst and six text evaluators was curated to reflect the dynamics of a training unit, where the text evaluators underwent supervision and training for system evaluation by the expert analyst trainer. Compensation was structured differently for each group: the expert analyst operated under an independent research contract, while each text evaluator received 20 USD per hour. 

%The intelligence analyst trainer had 10 years of experience in intelligence analyst training and intelligence tool evaluation, and was sourced through a partnership with an independent US-based national defense and security firm. 
%Next, six text analysts with advanced degrees in Computer Science (ranging from Bachelors to PhDs) and at least a year of text annotation experience were recruited. These included three natural language processing graduate students and three computer science undergraduate students, all fluent in English and based in the US. The recruitment of the single intelligence analyst trainer and six text analysts was curated to reflect a trained unit dynamic, where the text analysts underwent supervision and training by the intelligence analyst trainer for the system evaluation. Compensation was structured differently for each group: the intelligence analyst operated under an independent research contract, while each text analyst received 20 USD / hour. 

\subsection{Readability Study}
\label{sec:readability_study}

\subsubsection{Baselines}

\textsc{SmartBook} leverages question-driven claim extraction (as described in \S{\ref{sec:smartbook}}) to pinpoint relevant information, from which it then generates the final summary. For baseline comparisons, we consider two alternatives. One is a \textit{query-focused summarization} baseline that takes the news articles as input directly (no extraction) and uses a large language model (LLM) to generate a query-focused summary\footnote{We use the same model to generate SmartBook and query-focused summaries. The prompt used is the same as in the summary generation example in Figure \ref{fig:overall_workflow}, except the entire news article texts are passed as context.}. This baseline's query here corresponds to the \textsc{SmartBook}'s strategic question. 
Further, since \textsc{SmartBook} uses news articles that are relevant to the event as the background corpus, we also compare it against a second web search + LLM baseline, using the web as the background corpora, first obtaining relevant web pages from internet search and then summarizing them using a large language model. This second baseline simulates a competitive strategy of directly obtaining information from an LLM-enabled web search engine\footnote{Specifically, we leverage \href{https://www.perplexity.ai}{perplexity.ai}, which combines web-search with LLM summarization. The query used is the strategic question, along with a phrase ``\textit{with respect to the Ukraine-Russia crisis between $<$timeline$>$}'' to ground the query.} (the \textit{web search + LLM} baseline is similar to a Bing search + a ChatGPT query for summary). We randomly selected summaries for 50 of \textsc{SmartBook}'s strategic questions to perform the readability evaluation.

\subsubsection{Study Setup}

For each generated summary, three text evaluators are asked to assess in terms of coherence, relevance, and usefulness with the scores ranging from 1 (worst) to 5 (best). For coherence and relevance, we follow the guidelines as in \cite{fabbri2021summeval}. Simply, \textit{coherence} measures the quality of all summary sentences collectively regardless of the question. \textit{Relevance} quantifies whether the summary contains key points that answer the given question. We define \textit{usefulness} as an indication of whether the summary provides non-trivial and insightful information for analysts, and suggests the breadth and depth of the provided key points. 

\input{tables/sum_human}
\input{tables/summaries_comparison}

\subsubsection{Results}
%\input{tables/sum_human}

Table~\ref{tab:sum_human} shows the results from the evaluation study of the summaries. We observe that SmartBook outperforms alternative competitive strategies on coherence, relevance, and usefulness. The benefit of our question-driven claim extraction step can be seen from the considerably more relevant summaries within SmartBook, compared to the direct query-focused summarization of the news articles without an explicit extraction step (row (3) vs (1)). Further, we see that directly obtaining information from the internet can give less useful content compared to the focused news-driven summarization within \textsc{SmartBook} (row (2) vs (3)). A set of summary examples is shown in Table \ref{tab:summaries_comparison}.
This evaluation demonstrates across the metrics that \textsc{SmartBook} provides valuable content in its summaries and outperforms the two baselines lacking an extraction step. 

\subsection{Editing Study}
\label{sec:editing_study}

\subsubsection{Study Setup}
% Revise to make it read like more a basic evaluation setup.

 The study was conducted with the expert analyst. As an initial exercise, the expert analyst was provided with 5 strategic questions from \textsc{SmartBook} and wrote summaries without the assistance of AI-assisted tools in the report generation. Following this, the analyst was encouraged to actively explore the features of \textsc{SmartBook}. The analyst was provided with 94 randomly sampled summaries from SmartBook-generated situation reports, and was asked to edit them till their content was acceptable as a professional report from an intelligence analyst. The \textsc{SmartBook} interface to the summaries were provided, and the analyst completed edits in a text editing software of their choice.

\subsubsection{Results}
\label{sec:first_draft}
%\input{tables/summaries_comparison}

 Given the revised summaries from the expert analyst, we aimed to measure the extent to which they made changes to the original summary content. Specifically, these edits were quantified in the form of (a) commonly used token-overlap-based metrics such as BLEU [51] and ROUGE [38] scores, and (b) Levenshtein edit distance [47], which measures the character-level changes required to transform the original summary to the revised summary. %These analyses were completed across all 94 randomly sampled summaries from SmartBook. 
Empirical results indicate that token overlap between generated and post-edited texts were high, with BLEU and ROUGE-L scores respectively at 59.0\% and 74.1\%. These metrics suggest that the generated reports from SmartBook are of sufficiently good-quality, such that extensive human expert revision may not be necessary. However, we acknowledge that a gap still exists between the automatically generated and human expert summary curation, as the Levenshtein edit distance computed at the character level is 34.4\%. Interestingly, 15\% of generated summaries were determined to be perfect, with no edits made by the expert analyst. 

Next, we examined how the edits were made. The general observation was that more content was inserted than was deleted by the expert analyst. The percentage of tokens inserted was 49.6\%, whereas the percentage of tokens deleted was only 2.3\%, suggesting that automated summary generation may generally need to be more detailed. 
While investigating the efficacy of SmartBook as an AI-assisted tool, the expert analyst reported: 

\begin{quote}
"Pointing out to individual claims, while possible, can be hard sometimes since you will be abstracting information across multiple claims." and that "SmartBook saves time." (SA1)
\end{quote}


%By quantitatively and qualitatively measuring the expert analyst's interaction with SmartBook, we understand that it acts a collaborative partner for situation report generation.
\input{tables/table2}
Table \ref{tab:human_edits} shows an example of edits (in color) made by an expert analyst for a machine-generated summary in SmartBook. We can see here that the human analyst added additional tactical information (in blue) to elaborate on certain aspects (e.g. what is special about the ``kamikaze'' type of drone). Further, the analyst can also added some interesting insights (in green) based on the information in the summary. Overall, this shows that \textsc{SmartBook} provides a good starting point for analysts to expand upon for the generation of situation reports. 

%{\textcolor{red}{\textbf{I am NOT seeing any green in Table 5. Was this lost somehow in creating it? if it cannot be found, then the caption should be adjusted and one sentence in the last paragraph, starting with "Further,..." should be dropped  -- Clare}}}

\subsubsection{Error Analysis}
\label{sec:error_analysis}
As noted in \S{\ref{sec:first_draft}}, it is noteworthy that 15\% of summaries produced by \textsc{SmartBook} needed no modifications, highlighting its proficiency in creating acceptable reports in some scenarios without human intervention. This suggests that as technology advances and iterative refinements are applied, this rate will likely improve, reducing the workload for analysts in the future. 
To gain a better understanding of the different types of errors in the remaining summaries, we asked the expert analyst to categorize the errors within them. The analyst was also shown the strategic question and the corresponding extracted contexts that were used to automatically generate the summary. The summary errors were categorized as follows:

\begin{itemize}
    \item \textit{No relevant contexts:} None of the extracted contexts are relevant to the question (and thereby the summary is expected to be fully irrelevant too).
    \item \textit{Inaccurate information in summary:} Summary has incorrect information, that is not reflective of the underlying input contexts.
    \item \textit{Incoherent summary:} Summary is incomprehensible and unclear.
    \item \textit{Incomplete summary:} Important information in the input contexts is missing in the summary.
    \item \textit{Irrelevant information in summary:} Summary has material that is not relevant to the question, despite some extracted contexts being relevant.
\end{itemize}

\begin{wrapfigure}{r}{0.4\linewidth}
\vspace{-2em} 
        \centering
        \includegraphics[width=0.85\linewidth]{figures/error_categories.png}
        \caption{Distribution of different error categories for the summaries within SmartBook.}
        \label{fig:error_cat} 
        \vspace{-1em} 
\end{wrapfigure}

Figure \ref{fig:error_cat} shows the distribution of error categories for the summaries. It can be seen that incompleteness of summaries is a predominant error, with more than 50\% of the summaries missing important information or not being sufficiently complete.  While the predominance of incomplete summaries could be a concern, this can also be framed positively: it represents a conservative approach ensuring that \textsc{SmartBook} does not over-extend based on limited data, and instead offers a foundational understanding.  Other errors corresponded to summaries with inaccurate (18.6\%) or irrelevant (14.6\%) information. Very few summaries were judged incoherent, as expected given that large language models such as GPT-3 have been shown \cite{goyal2022news, zhang2023benchmarking} to generate fluent and easy-to-read output. 




==> sections/9_Discussion.tex <==
\section{Discussion}
%Intelligence is more than data aggregation and hypothesis formation.


% In this direction, we study whether SmartBook-generated situation reports can be a useful preliminary draft, in comparison to intelligence analysts' prior experience in solely authoring situation reports.


 %This leaves room for human analysts to augment and fine-tune, merging AI's broad processing capacity with human expertise.

%\revanth{As per Agathe's feedback, this section needs to have a broad high-ranging discussion of the results and potential impact of this work.}
%\textcolor{blue}{SmartBook provides a reliable, accurate, and efficient method for digesting a complex and large corpus of news and thus also supports a wide-open vision for a new approach to the authoring of situation reports, as well as the vast range of summary reports in the business world (\ref{sec:outlook}). Our approach to the development of SmartBook represents an application of the ``research-through-design'' methodology within AI design, a strategy not widely explored in this domain. This approach offers a pragmatic, real-world setting for human-AI collaboration, by emphasizing the tangible needs of practitioners, in this case intelligence analysts and decision makers. Consequently, SmartBook stands as a significant exemplar of how AI can be effectively rooted in addressing specific, practical challenges, thus making a remarkable contribution to both Human-Computer Interaction (HCI) and AI disciplines.}

SmartBook leverages the zero-shot capabilities~\cite{brown2020language} of LLMs for tasks with limited training data. Complex tasks like grounded summary generation with citations and strategic question identification are tackled by LLMs, while smaller models address well-defined tasks with available data, such as event headline (chapter name) generation~\cite{headline2020}, duplicate question detection~\cite{cer2017semeval}, and claim extraction through question answering~\cite{kwiatkowski2019natural}. Our experiments revealed a tendency of the LLMs to generate similar strategic questions, necessitating sampling methods~\cite{holtzman2019curious} for variety. Directing the LLMs to reference input documents while generating summaries enhanced factuality, aligning with recent findings~\cite{gao-etal-2023-enabling}. Nevertheless, LLMs' tendency to hallucinate~\cite{ji2022survey, tam2022evaluating}, evident from inaccuracy errors in \S{\ref{sec:error_analysis}}, necessitates future enhancements  in validation and cross-referencing techniques (discussed in \S{\ref{sec:future_verification}}) to mitigate this issue.


In light of the ongoing developments in AI-assisted writing~\cite{WangACL2019,Wang2020,selfcollaboration2023,cardon2023challenges}, where tools have been developed for a variety of end-users like academics~\cite{gero2022sparks}, screenwriters~\cite{mirowski2023co} and developers~\cite{chen2021evaluating}, SmartBook introduces a unique automated framework designed specifically for generating situation reports for intelligence analysts. Prior AI-assisted writing systems, such as CoAuthor~\cite{lee2022coauthor}, Creative Help~\cite{roemmele2015creative}, Writing Buddy~\cite{samuel2016design} and WordCraft~\cite{yuan2022wordcraft}, are designed to be collaborative and aid in creative tasks~\cite{klein1973automatic}. SmartBook highlights a different aspect of human-AI collaboration, where AI's role is more about efficient information processing with analytical rigor and less about creative or iterative human engagement. This distinction underscores SmartBook's design with a focus on factuality, analytical depth, and efficiency in more structured, data-driven environments, such as intelligence analysis. Clearly the design also stands to benefit from iterative experimentation and refinement, to explore where deeper integration of SmartBook into analysts' workflows improve their task performance. We discuss this as future extensions in \S{\ref{sec:iterative_refinement}}.


\subsection{Outlook}
\label{sec:outlook}
%\textcolor{blue}{\textbf{TODO: Daniel - Connect brief overview of what were our takeaways / understandings (based on formative study) of how analysts originally perceived AI generated outputs, and how they were using SmartBook reports in the studies. Discussion should be high-level and ideally not repeat anything that was mentioned in results of the formative study/user study.}}

The central challenge faced by analysts is massive data overload that they must filter in addressing information requirements to produce situation reports.  The key findings of the formative study show that analysts, though appropriately cautious, are open to incorporating AI assistance into their workflow.  The desiderata in the design strategies that they articulated during the collaborative design also make clear that they are eager to participate in crafting the new vision that will include AI assistance that not only adjusts to the data content of shifting scenarios but also to their individual analytic methods.

SmartBook, characterized by its generalizable and modular design, can efficiently automate the generation of situation reports across various scenarios, including geopolitical, environmental, or humanitarian contexts. Unlike human analysts who face considerable challenges in transferring their expertise across domains, SmartBook requires minimal configuration for such shifts. This transition in traditional settings involves extensive background research and the recruitment of domain experts, demanding substantial time and effort. Furthermore, each new scenario introduces complex variables and details that must be meticulously integrated. SmartBook addresses these challenges with a streamlined and consistent approach, thereby offering accurate reports in diverse and rapidly changing global contexts.

The effectiveness of SmartBook was primarily evaluated on news articles from the Ukraine-Russia military conflict. Here, we briefly explore SmartBook's applicability in a humanitarian crisis, specifically the Turkey-Syria earthquake. By changing the source articles\footnote{Here is a URL corresponding to news for February 6: \href{https://edition.cnn.com/middleeast/live-news/turkey-earthquake-latest-020623/index.html}{link}} for major event identification, SmartBook successfully generated pertinent situation reports for the specified time window (February 6-13). These reports accurately captured critical aspects of the earthquake disaster, such as aftershock impacts (\href{https://www.cnn.com/middleeast/live-news/turkey-syria-earthquake-updates-2-7-23-intl/h_a9e1d082dd54c67187fd51322f95eaf2}{link}), international humanitarian assistance (\href{https://www.incirlik.af.mil/News/Article-Display/Article/3292036/urban-search-and-rescue-teams-arrive-at-incirlik-air-base/}{link}), rising death tolls (\href{https://www.reuters.com/world/middle-east/death-toll-syria-turkey-quake-rises-more-than-8700-2023-02-08/}{link}), and specific events like the disappearance of a Ghanaian soccer star (\href{https://www.marketwatch.com/story/soccer-star-christian-atsu-still-missing-after-turkey-earthquakes-i-still-pray-and-believe-that-hes-alive-says-partner-cfd47272}{link}). 

This adaptability of SmartBook, demonstrated in the domain shift from military to humanitarian crisis contexts, underscores its robustness and versatility. It also emphasizes the importance of the source articles and suggests that, with mission-relevant data input, SmartBook has the potential to be an invaluable tool for analysts across a multitude of scenarios. Overall, SmartBook presents an exciting step forward in AI-assisted situation report generation and signifies a momentous stride in the domain of intelligence analysis.



%\textcolor{blue}{In this section, we describe some key learnings and implications of this project (in \S{\ref{sec:learnings}}) both from the perspective of HCI+AI and intelligence analysis communities. Next, we discuss explorations (in \S{\ref{sec:transferability}}) for applying SmartBook to scenarios in other intelligence domains . Finally, we highlight some limitations of SmartBook (in \S{\ref{sec:limitations}}) and present directions for future work (in \S{\ref{sec:extensions}}).}

%Given the surprisingly high-performance zero-shot capabilities of LLMs, SmartBook leverages LLMs for tasks without considerable training data, such as grounded summary generation with citations, and identifying strategic questions. On the other hand, smaller models were leveraged for focused tasks that had training data available, such as event headline (chapter name) generation~\cite{headline2020}, duplicate question detection~\cite{cer2017semeval}, and claim extraction using question answering~\cite{kwiatkowski2019natural}. From our experiments, we observed that even when prompted to generate diverse strategic questions, the model was prone to generating very similar ones, thereby requiring sampling tricks and repeated generation to promote variety. In addition, initial explorations suggested that specifically instructing the language model to cite input documents improved the factuality of the generated summaries, as evidenced in recent works~\cite{gao-etal-2023-enabling}.However, the hallucination problem \cite{ji2022survey, tam2022evaluating} of such LLMs is evident from the considerable number of summaries (in \S{\ref{sec:error_analysis}}) with inaccurate information. This could be mitigated in future iterations (as discussed in \S{\ref{sec:future_verification}}) by incorporating stronger validation mechanisms and cross-referencing techniques.} 


%AI-assisted writing~\cite{WangACL2019,Wang2020,selfcollaboration2023,cardon2023challenges} is a rapidly growing field in human-computer interaction research. In recent years, researchers have explored various approaches to develop AI systems that can assist users in writing tasks. AI-assisted writing tools have demonstrated benefits to a variety of end-users, like academics~\cite{gero2022sparks}, screenwriters~\cite{mirowski2023co} and developers~\cite{chen2021evaluating}. CoAuthor~\cite{lee2022coauthor} crafts a dataset that encapsulates the rich interactions observed between multiple writers and instances of GPT-3 over numerous writing sessions, thereby highlighting the efficacy of AI in fostering collaborative writing endeavors. In the area of automated story-writing~\cite{klein1973automatic}, attempts such as Creative Help~\cite{roemmele2015creative}, Writing Buddy~\cite{samuel2016design} and WordCraft~\cite{yuan2022wordcraft} aid the user in producing full stories with creative control throughout the process. More recently, with humans struggling to identify text as being machine generated ~\cite{wahle2022large}, concerns have been raised about academic integrity~\cite{perkins2023academic} and plagiarism\cite{wahle2022identifying} when using AI-assisted writing tools.In light of the ongoing developments in AI-assisted writing, SmartBook introduces a unique automated framework designed specifically for generating situation reports for intelligence analysts. While the existing body of work predominantly focuses on augmenting creative and collaborative writing, SmartBook aims to assist intelligence analysts' workflows with a focus on factuality and analytical depth.

%Qualitative evaluations underscore the potent functionality of SmartBook, with a significant majority of its automatically discovered questions directing focus on strategic information. Additionally, in addressing the current geopolitical tensions in the Ukraine-Russia context, it has demonstrated its indispensability in strategizing and planning, showcasing not only its adaptability to real-world scenarios but also its capacity to provide actionable intelligence. }


%\subsection{Implications}

%\textcolor{blue}{ Firstly, it is noteworthy that 15\% of summaries produced by SmartBook needed no modifications, highlighting its proficiency in creating acceptable reports in some scenarios without human intervention. This suggests that as technology advances and iterative refinements are applied, this rate could potentially increase, reducing the workload for analysts even further.  Lastly, the hallucination problem, although present, could be mitigated in future iterations (which we discuss in Section \ref{sec:future_verification}) by incorporating stronger validation mechanisms and cross-referencing techniques.}


%\subsection{Implications}


%SmartBook emphasizes generalizability in automating the generation of situation reports. Its modular design ensures that when the need arises to transition to a new scenario - be it geopolitical, environmental, or humanitarian - SmartBook can adapt with minimal configuration. Meanwhile, traditional intelligence analysts often grapple with a multifaceted challenge when pivoting between scenarios. The transition demands a significant time investment for deep dive into background research, recruitment of domain experts, etc. Additionally, each new scenario introduces a vast array of variables and particulars that need to be meticulously accounted for and incorporated. The inherent cognitive constraints on an individual analyst's capacity to process and synthesize vast amounts of information mean that the risk of oversight or error is always present. In stark contrast, SmartBook offers a streamlined, consistent, and efficient mechanism to adapt and provide accurate situation reports across diverse scenarios in rapidly changing global contexts. %This makes it an invaluable asset in rapidly changing global contexts, ensuring timely and reliable generation of situation reports.

 %We evaluated SmartBook primarily in the context of a military conflict by choosing Ukraine-Russia crisis as the evaluation scenario. In this section, we explore the possibility of how well SmartBook can generalize to intelligence analysis for a humanitarian crisis. Specifically, we consider situation report generation for the Turkey-Syria earthquake scenario by considering a single timeline for the time window of February 6 - 13. This aims to demonstrate portability to new scenarios, by simply switching the source articles\footnote{Here is a URL corresponding to news for February 6: \href{https://edition.cnn.com/middleeast/live-news/turkey-earthquake-latest-020623/index.html}{link}} used to identify major events (described on Section \ref{subsec:major_event}). We observe that SmartBook is able to identify and present important aspects of the Turkey-Syria earthquake disaster, such as the continued impact of aftershocks (\href{https://www.cnn.com/middleeast/live-news/turkey-syria-earthquake-updates-2-7-23-intl/h_a9e1d082dd54c67187fd51322f95eaf2}{link}), international humanitarian assistance in the form of search and rescue teams (\href{https://www.incirlik.af.mil/News/Article-Display/Article/3292036/urban-search-and-rescue-teams-arrive-at-incirlik-air-base/}{link}), the rising death toll in the aftermath of the earthquake (\href{https://www.reuters.com/world/middle-east/death-toll-syria-turkey-quake-rises-more-than-8700-2023-02-08/}{link}) and missing of a soccer star from Ghana (\href{https://www.marketwatch.com/story/soccer-star-christian-atsu-still-missing-after-turkey-earthquakes-i-still-pray-and-believe-that-hes-alive-says-partner-cfd47272}{link}). The results from the Turkey-Syria earthquake scenario indicate that SmartBook's underlying framework is adaptable and effective across diverse situation report contexts. The ability to transition from a military conflict to a humanitarian crisis, while maintaining accuracy in capturing key events, highlights robustness and versatility. It also emphasizes the importance of the source articles and suggests that with the right data input, SmartBook has the potential to be an invaluable tool for analysts across a multitude of scenarios.


\subsection{Limitations}
\label{sec:limitations}
While SmartBook represents a significant advancement in the automated generation of situation reports, it is essential to acknowledge certain limitations that stem from both the technical aspects of the system and the scope of its application. These include unverified news source credibility, potential inaccuracies in reflecting source material despite citations, and user studies focused mainly on military intelligence analysts, which may not represent the needs of a wider analytical audience. Recognizing these limitations is crucial for guiding future improvements and ensuring the framework's applicability across across diverse intelligence and analysis sectors.

\begin{itemize}
    %\item \textcolor{blue}{In addressing the capabilities of SmartBook, it is important to clarify that its current functionalities are directed towards the goal of providing a comprehensive initial draft of situation reports. SmartBook currently does not support multi-turn editing or the iterative refinement of reports. In its role as an initial draft provider to streamline the early stages of situation report generation, SmartBook is intended to be a valuable aid in the intelligence analysis workflow, though not as a standalone solution for the entire report development cycle.}
    \item The generation of situation reports within SmartBook leverages news articles aggregated from Google News. Nonetheless, the process does not involve a rigorous assessment of the news sources' credibility, nor does it incorporate an explicit verification of the factual accuracy of the claims used in the summary generation model. Considering the extensive exploration of these aspects within computational social science~\cite{lee2023pandemic} and natural language processing~\cite{gong2023fake}, we deemed them beyond the scope of SmartBook's framework in this work.
    \item SmartBook enhances the reliability and credibility of the generated situation reports by incorporating citations. However, it does not rigorously ensure the accuracy of these reports in reflecting the content of the source documents.
     In contrast, LLMs have been shown~\cite{mallen2022not, baek2023knowledge} to tend to produce content that may not directly correlate to the source materials. While this is still an active area of research, recent studies~\cite{tian2023fine} have shown that LLMs can be effectively optimized to enhance factual accuracy and attribution capabilities~\cite{gao2023enabling}. Consequently, we propose that future advancements could involve substituting the current summary-generating language model with one that is specifically refined for improved attribution~\cite{gao2023enabling}.%{While SmartBook helps promote trust and credibility of the generated situation reports through the addition of citations, it does not explicitly verify the faithfulness of the generated reports to the input documents. On the other hand, LLMs can generate content that is not attributable~\cite{} to input documents. While this is still an active area of research, recent work~\cite{} has demonstrated that large language models can be specifically tuned to improve factuality and the ability to attribute. Therefore, we assert that this can be tackled in future work by replacing the language model generating the summaries with a model fine-tuned for attribution.}
    \item The selection of analysts for the user studies in SmartBook was primarily comprised of individuals from military intelligence. This limitation arose due to the challenges encountered in recruiting analysts who could participate without breaching confidentiality agreements. Consequently, our recruitment efforts were confined to analysts within our existing networks. It is important to recognize that our studies may not fully represent the needs and perspectives of analysts in other fields, such as political, corporate, or criminal analysis. Acknowledging this gap, future work can aim to extend and adapt SmartBook's capabilities for generating situation reports, tailoring them to meet the distinct requirements of each of these domains.%{The analysts recruited for the user studies in SmartBook are predominantly military analysts. This stems from the difficulty in recruiting analysts given confidentiality agreements, hence we were restricted to recruiting those based on prior connections. However, we acknowledge that our studies do not account for other domains such as political analysis, corporate analysis, or criminal analysis. We leave this for future work, to expand and customize SmartBook's formulation of situation report generation to the specific requirements for each of these domains.}
\end{itemize}

\subsection{Future Extensions}
\label{sec:extensions}
This section outlines key extensions planned for SmartBook, each aiming to enhance its functionality and utility. SmartBook's future enhancements include integrating multimodal and multilingual information to enrich intelligence analysis (in \S{\ref{sec:multimodal_info}}) and employing a balanced approach to news sources to mitigate biases (in \S{\ref{sec:source_bias}}). Additionally, the system will evolve with a co-authoring feature for dynamic report refinement (in \S{\ref{sec:iterative_refinement}}) and introduce a `verification score' to assess the reliability of claims, ensuring precise and dependable decision-making support (in \S{\ref{sec:future_verification}}). Overall, these extensions are designed to elevate SmartBook's utility as a comprehensive, bias-balanced, and reliable tool for situation report generation in intelligence analysis.


\subsubsection{Incorporating Multimodal, Multilingual Information:}
\label{sec:multimodal_info} %In intelligence analysis, situation reports often integrate diverse data types, including textual accounts, news articles, photographs, videos, and audio recordings, each offering unique insights. Figure \ref{fig:multimodal_example} illustrates how images can corroborate or challenge textual evidence in SmartBook, highlighting the value of multimodal data. We aim to enhance SmartBook's comprehensiveness by integrating various data modalities, correlating textual claims with pertinent multimedia elements using advanced multimedia knowledge extraction systems such as GAIA~\cite{li2020gaia}. This integration envisions an ecosystem where AI-assisted report generation merges multiple data types, providing analysts a comprehensive, nuanced, and corroborated narrative.\\
 Intelligence analysis increasingly requires the integration of diverse data types, including text, images, videos, and audio recordings, to provide a comprehensive understanding of global events. We plan to enrich SmartBook's situation reports by correlating textual claims with relevant multimedia elements, leveraging systems like GAIA~\cite{li2020gaia} for advanced multimedia knowledge extraction. Figure \ref{fig:multimodal_example} exemplifies how images can support or contradict the text, underscoring the value of incorporating various data modalities. In addition to multimodal data, the globalization of events necessitates a multilingual approach to intelligence analysis, as reliance on English alone can overlook critical local nuances. SmartBook aims to overcome this limitation by incorporating multiple languages, enabling a more profound understanding of local dynamics that influence global situations, capturing cultural subtleties, regional politics, and localized social phenomena in native languages. Moreover, integrating multilingual sources democratizes intelligence analysis, moving beyond a predominantly English-speaking worldview. Ultimately, SmartBook seeks to redefine intelligence reporting standards, promoting a more inclusive and globally aware approach.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/multimodal_example.png}
    \caption{Figure showing an example of how multimodal information (in the form of images) supports and provides additional context to the claims presented in SmartBook. In this example, the presence of anti-aircraft weapons (as seen in the image) in Ukraine provides background for the discussion in NATO on whether to impose a no-fly zone.}
    \label{fig:multimodal_example}
\end{figure}

    \subsubsection{Controlling the Bias of News Sources:} \label{sec:source_bias} Different news sources inevitably bring with them biases that stem from factors such as editorial policies, audience demographics, and geographical influences. When a single news source or perspective dominates the narrative, key details or alternative viewpoints can be easily missed. In our vision for the next iteration of SmartBook, we aim to address these inherent biases. To overcome such challenges, it is essential to source information from a diverse array of news outlets, encompassing left-leaning, centrist, and right-leaning perspectives. %This strategy enables SmartBook to facilitate the recognition of various hypotheses and interpretations of events. 
    The goal is to enhance SmartBook's utility for intelligence analysts by reducing informational blind spots and broadening the range of considered scenarios.
%Different news sources present information from varying angles, with different levels of detail and interpretation. Thereby, we plan to control for the bias of news sources used in the creation of SmartBook to help cross-check information and avoid the potential pitfalls of relying on a single news source or a single interpretation of events. Further, alternate perspectives/hypotheses can be identified by independently considering news sources on the left, in the center, and on the right. \\
    %\item \textbf{Controlling the bias of sources}: To control bias in SmartBook, we will cross-check information from various news sources with differing angles, levels of detail, and interpretations, and also consider independent sources from the left, center, and right to identify alternate perspectives and hypotheses. \\

    \subsubsection{Co-Authoring with Iterative Refinement:} \label{sec:iterative_refinement} Authoring situation reports is an iterative process where analysts continuously refine and update the reports. In the next iteration, we aim to incorporate advanced co-authoring capabilities that will enable intelligence analysts to engage with SmartBook in a dynamic, multi-turn editing process. By integrating machine learning algorithms for continual learning~\cite{lopez2017gradient, zenke2017continual} and personalization~\cite{wu2019npa, monzer2020user}, SmartBook can learn from each interaction to progressively adapt to the analysts' preferences and decision-making styles. Further, recent techniques like Reinforcement Learning with Human Feedback (RLHF)~\cite{stiennon2020learning, bai2022training} can enable the system to assimilate human feedback, thereby refining its understanding of analysts' editing and reasoning patterns.
%can enable the system to analyze changes and feedback provided by human analysts, allowing it to understand and replicate the nuances of their editing and reasoning processes. 
This approach aims to improve SmartBook's alignment with human decisions over time and help generate reports that are tailored to the specific needs of intelligence analysis workflows. %This learning mechanism will not only improve SmartBook's alignment with human decisions over time, but also ensure that the generated reports are increasingly are relevant, and tailored to the specific needs of intelligence analysis workflows. 
     As a result, SmartBook will evolve from a preliminary drafting tool to a comprehensive AI co-author for generating situation reports.

    %\subsubsection{Adding More Languages} In an era of globalization, events that transpire in one part of the world often ripple out and influence other regions. While English remains a dominant language for international news, relying solely on it can lead to a narrowed viewpoint, potentially missing local nuances and sentiments. By integrating more languages, SmartBook seeks to transcend these linguistic barriers, enhancing the depth and breadth of the intelligence analysis. Furthermore, the integration of multilingual sources will be a critical step towards facilitating a deeper comprehension of intricate local dynamics that influence global situations. Cultural nuances, regional politics, and localized social phenomena are often best captured in native languages, offering unfiltered and nuanced insights that might be lost or distorted in translation. Additionally, this expansion promises to foster a more inclusive approach where information is not monopolized by predominantly English-speaking perspectives, thereby democratizing the intelligence analysis process. Through this endeavor, SmartBook aspires to set a new benchmark in intelligence reporting, championing a more inclusive, empathetic, and globally conscious approach.
    
    %The world is diverse, and news articles from different languages allow capturing different perspectives, insights, and information relating to global events, that might not be available in a single language. For this reason, we aim to add news articles from more languages into SmartBook to present a more comprehensive and accurate picture. Further, the ability to ingest information from different languages also enables analysts to understand local customs, cultures, and nuances that may influence the interpretation of events.\\   
    \subsubsection{Verifying the extracted claims:}\label{sec:future_verification} The integrity of data and claims in situation reports is crucial for strategic decision-making. A key challenge in automating these reports is guaranteeing the accuracy and reliability of extracted data from extensive sources. To address this, we plan to introduce a `verification score' for each claim. This score assesses the reliability of information, considering factors like source credibility, corroborative data, and historical accuracy of similar claims. It provides a confidence metric for intelligence analysts, aiding in swift evaluation of data reliability. High scores enhance confidence and facilitate quick integration into reports, while low scores signal the need for thorough review and potential further verification. This blend of automation and human oversight is essential to ensure the effectiveness of SmartBook's situation reports in strategic planning.
    %Given that situation reports contribute towards strategic planning, it is important to present accurate information to prevent misguided decisions and actions. Hence, we intend to provide a verification score, for each claim presented within SmartBook, which can be interpreted as a measure of trustworthiness. Claims with lower scores signal the need for additional oversight by the intelligence analysts before incorporating into them the final report.
    %\item \textbf{Verifying the extracted claims}: Since situation reports inform strategic planning, we will provide a trustworthiness verification score for each SmartBook claim to ensure accuracy and prevent misguided actions, with lower scores indicating the need for further analyst oversight before final report inclusion.
%\end{itemize}

==> tables/system_eval_demographic.tex <==
\begin{table}[]
\centering
\label{tab:participants}
%\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{PID} &
  \textbf{Age} &
  \textbf{Education} &
  \textbf{Analyst Training Exp.} &
  \\\midrule
AT1 & 25-34 & Bachelor's & 5 - 10 years & 2 & Rarely \\
    \midrule
    \textbf{PID} &
    \textbf{Age} &
    \textbf{Education} &
    \textbf{Text Annotation Exp.} &
    \\\midrule
DA1 & 25-34 & Bachelor's & 2 - 5 years & 1 & Rarely  
DA2 & 25-34 & Bachelor's & 2 - 5 years & 1 & Rarely  
DA3 & 25-34 & Bachelor's & 2 - 5 years & 1 & Rarely  
DA4 & 25-34 & Bachelor's & 2 - 5 years & 1 & Rarely  
DA5 & 25-34 & Bachelor's & 2 - 5 years & 1 & Rarely  
DA6 & 25-34 & Bachelor's & 2 - 5 years & 1 & Rarely  
\\ 
\bottomrule      
\end{tabular}
\vspace{0.3em}
\caption{\textcolor{blue}{Demographic information of formative study participants who are experienced in intelligence report generation.}}
\end{table}
